Multi-tier Caching Analysis in CDN-based Over-the-top Video Streaming Systems

Internet video traffic has been been rapidly increasing and is further expected to increase with the emerging 5G applications such as higher definition videos, IoT and augmented/virtual reality applications. As end-users consume video in massive amounts and in an increasing number of ways, the content distribution network (CDN) should be efficiently managed to improve the system efficiency. The streaming service can include multiple caching tiers, at the distributed servers and the edge routers, and efficient content management at these locations affect the quality of experience (QoE) of the end users. In this paper, we propose a model for video streaming systems, typically composed of a centralized origin server, several CDN sites, and edge-caches located closer to the end user. We comprehensively consider different systems design factors including the limited caching space at the CDN sites, allocation of CDN for a video request, choice of different ports (or paths) from the CDN and the central storage, bandwidth allocation, the edge-cache capacity, and the caching policy. We focus on minimizing a performance metric, stall duration tail probability (SDTP), and present a novel and efficient algorithm accounting for the multiple design flexibilities. The theoretical bounds with respect to the SDTP metric are also analyzed and presented. The implementation on a virtualized cloud system managed by Openstack demonstrate that the proposed algorithms can significantly improve the SDTP metric, compared to the baseline strategies.

==> abstract.tex <==
\begin{abstract}
Traffic for Over-the-top video streaming has been rapidly increasing. The traffic is further expected to increase with the higher definition videos and augmented reality applications. This necessitates efficient management of different cloud resources to optimize the quality of experience of the end users. This paper considers a CDN-based video streaming system where the cache at the CDN, allocation of CDN for a video request, choice of different ports from the CDN and the central storage, bandwidth allocation are all variables that can be decided. A novel two-stage probabilistic scheduling policy is proposed, and bounds for the stall duration tail probability are derived. A holistic optimization framework is developed to optimize a weighted user experience of all video files over the request scheduling probabilities, cache content placement, the bandwidth allocation among different streams,  and the modeling parameters in the bound. Efficient algorithm to solve the problem is proposed. The  experimental results demonstrate significant improvement in the QoE metric  as compared to the considered baseline strategies.
\end{abstract}







==> apdx_algs.tex <==
%\section{Algorithm Pseudo-codes for the Sub-problems}\label{apdx_table}


\begin{algorithm}[t]
\caption{NOVA Algorithm to solve Server Access and PSs selection Optimization sub-problem\label{alg:NOVA_Alg1Pi}}

\begin{enumerate}
\item \textbf{Initialize} $\nu=0$, $k=0$,$\gamma^{\nu}\in\left(0,1\right]$,
$\epsilon>0$,$\widetilde{\boldsymbol{\pi}}^{0}$ such that $\widetilde{\boldsymbol{\pi}}^{0}$
is feasible ,
\item \textbf{while} $\mbox{obj}\left(k\right)-\mbox{obj}\left(k-1\right)\geq\epsilon$
\item $\quad$//\textit{\small{}Solve for $\widetilde{\boldsymbol{\pi}}^{\nu+1}$ with
given $\widetilde{\boldsymbol{\pi}}^{\nu}$}{\small \par}
\item $\quad$\textbf{Step 1}: Compute $\boldsymbol{\widehat{\pi}}\left(\widetilde{\boldsymbol{\pi}}^{\nu}\right),$
the solution of $\boldsymbol{\widehat{\pi}}\left(\widetilde{\boldsymbol{\pi}}^{\nu}\right)=$$\underset{\widetilde{\boldsymbol{\pi}}}{\text{argmin}}$
$\boldsymbol{\widetilde{U}}\left(\widetilde{\boldsymbol{\pi}},\widetilde{\boldsymbol{\pi}}^{\nu}\right)\,\, $ s.t.
$\left(\eqref{eq:rho_beta_d}--\eqref{eq:pi_q_p_gz}\right)$, $\left(\eqref{eq:mgf_beta_d}--
\eqref{eq:mgf_beta_e}\right)$, solved using  projected gradient descent 



\item $\quad$\textbf{Step 2}: $\ensuremath{\widetilde{\boldsymbol{\pi}}^{\nu+1}=\widetilde{\boldsymbol{\pi}}^{\nu}+\gamma^{\nu}\left(\widehat{\boldsymbol{\pi}}\left(\widetilde{\boldsymbol{\pi}}^{\nu}\right)-\widetilde{\boldsymbol{\pi}}^{\nu}\right)}$.
\item $\quad$//\textit{\small{}update index}{\small \par}
\item \textbf{Set} $\ensuremath{\nu\leftarrow\nu+1}$
\item \textbf{end while}
\item \textbf{output: }$\ensuremath{\widehat{\boldsymbol{\pi}}\left(\widetilde{\boldsymbol{\pi}}^{\nu}\right)}$
\end{enumerate}
\end{algorithm}



\begin{algorithm}[ht]
	\caption{NOVA Algorithm to solve Auxiliary Variables  Optimization sub-problem\label{alg:NOVA_Alg1}}
	
	\begin{enumerate}
		\item \textbf{Initialize} $\nu=0$, $\gamma^{\nu}\in\left(0,1\right]$, $\epsilon>0$, $\boldsymbol{t}^{0}$ 
		such that $\boldsymbol{t}^{0}$  is feasible,
		\item \textbf{while} $\mbox{obj}\left(\nu\right)-\mbox{obj}\left(\nu-1\right)\geq\epsilon$
		\item $\quad$//\textit{\small{}Solve for  $\boldsymbol{t}^{\nu+1}$ with
			given $\boldsymbol{t}^{\nu}$}{\small \par}
		\item $\quad$\textbf{Step 1}: Compute $\boldsymbol{\widehat{t}}\left(\boldsymbol{t}^{\nu}\right),$
		the solution of  $\boldsymbol{\widehat{t}}\left(\boldsymbol{t}^{\nu}\right)=$$\underset{\boldsymbol{t}}{\text{argmin}}$
		$\boldsymbol{\overline{U}}\left(\boldsymbol{t},\boldsymbol{t}^{\nu}\right)$, s.t. \eqref{eq:t_leq_alpha_beta_d}--\eqref{eq:mgf_beta_e}, using projected gradient descent
\item $\quad$\textbf{Step 2}: $\ensuremath{\boldsymbol{t}^{\nu+1}=\boldsymbol{t}^{\nu}+\gamma^{\nu}\left(\widehat{\boldsymbol{t}}\left(\boldsymbol{t}^{\nu}\right)-\boldsymbol{t}^{\nu}\right)}$.
		\item $\quad$//\textit{\small{}update index}{\small \par}
		\item \textbf{Set} $\ensuremath{\nu\leftarrow\nu+1}$
		\item \textbf{end while}
		\item \textbf{output: }$\ensuremath{\widehat{\boldsymbol{t}}\left(\boldsymbol{t}^{\nu}\right)}$
	\end{enumerate}
\end{algorithm}



\begin{algorithm}[ht]
	\caption{NOVA Algorithm to solve Bandwidth Allocation Optimization sub-problem\label{alg:NOVA_Alg3}}	
	\begin{enumerate}
		\item \textbf{Initialize} $\nu=0$, $\gamma^{\nu}\in\left(0,1\right]$, $\epsilon>0$, $\boldsymbol{w}^{0}$ 
		such that $\boldsymbol{w}^{0}$  is feasible,
		\item \textbf{while} $\mbox{obj}\left(\nu\right)-\mbox{obj}\left(\nu-1\right)\geq\epsilon$
		\item $\quad$//\textit{\small{}Solve for  $\boldsymbol{w}^{\nu+1}$ with
			given $\boldsymbol{w}^{\nu}$}{\small \par}
		\item $\quad$\textbf{Step 1}: Compute $\boldsymbol{\widehat{w}}\left(\boldsymbol{w}^{\nu}\right),$
		the solution of  $\boldsymbol{\widehat{w}}\left(\boldsymbol{w}^{\nu}\right)=$$\underset{\boldsymbol{b}}{\text{argmin}}$
		$\boldsymbol{\overline{U}}\left(\boldsymbol{w},\boldsymbol{w}^{\nu}\right)$, s.t. \eqref{eq:w_cde_gz}--
\eqref{eq:sum_w_de},\,\,\eqref{eq:t_leq_alpha_beta_d}--\eqref{eq:mgf_beta_e}, using projected gradient descent
		\item $\quad$\textbf{Step 2}: $\ensuremath{\boldsymbol{w}^{\nu+1}=\boldsymbol{w}^{\nu}+\gamma^{\nu}\left(\widehat{\boldsymbol{w}}\left(\boldsymbol{w}^{\nu}\right)-\boldsymbol{w}^{\nu}\right)}$.
		\item $\quad$//\textit{\small{}update index}{\small \par}
		\item \textbf{Set} $\ensuremath{\nu\leftarrow\nu+1}$
		\item \textbf{end while}
		\item \textbf{output: }$\ensuremath{\widehat{\boldsymbol{w}}\left(\boldsymbol{w}^{\nu}\right)}$
	\end{enumerate}
\end{algorithm}






\begin{algorithm}[ht]
	\caption{NOVA Algorithm to solve Cache Placement Optimization sub-problem\label{alg:NOVA_Alg5}}
	
	\begin{enumerate}
		\item \textbf{Initialize} $\nu=0$, $\gamma^{\nu}\in\left(0,1\right]$, $\epsilon>0$, $\boldsymbol{L}^{0}$ 
		such that $\boldsymbol{L}^{0}$  is feasible,
		\item \textbf{while} $\mbox{obj}\left(\nu\right)-\mbox{obj}\left(\nu-1\right)\geq\epsilon$
		\item $\quad$//\textit{\small{}Solve for  $\boldsymbol{L}^{\nu+1}$ with
			given $\boldsymbol{L}^{\nu}$}{\small \par}
		\item $\quad$\textbf{Step 1}: Compute $\boldsymbol{\widehat{L}}\left(\boldsymbol{L}^{\nu}\right),$
		the solution of  $\boldsymbol{\widehat{L}}\left(\boldsymbol{L}^{\nu}\right)=$$\underset{\boldsymbol{L}}{\text{argmin}}$
		$\boldsymbol{\overline{U}}\left(\boldsymbol{L},\boldsymbol{L}^{\nu}\right)$, s.t. \eqref{eq:rho_beta_d}--
\eqref{eq:rho_nu_e},
\eqref{eq:capConst},
\eqref{eq:mgf_beta_d}-- \eqref{eq:mgf_beta_e}\\
		using projected gradient descent
		\item $\quad$\textbf{Step 2}: $\ensuremath{\boldsymbol{L}^{\nu+1}=\boldsymbol{L}^{\nu}+\gamma^{\nu}\left(\widehat{\boldsymbol{L}}\left(\boldsymbol{L}^{\nu}\right)-\boldsymbol{L}^{\nu}\right)}$.
		\item $\quad$//\textit{\small{}update index}{\small \par}
		\item \textbf{Set} $\ensuremath{\nu\leftarrow\nu+1}$
		\item \textbf{end while}
		\item \textbf{output: }$\ensuremath{\widehat{\boldsymbol{L}}\left(\boldsymbol{L}^{\nu}\right)}$
	\end{enumerate}
\end{algorithm}


==> bio.tex <==

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./bio/abubakr}}]{Abubakr O. Al-Abbasi (S'11)} received the B.Sc. and M.Sc. degrees in electronics and electrical communications engineering from Cairo University, Cairo, Egypt, in 2010, and 2014, respectively. He is currently pursuing the Ph.D. degree with Purdue University, USA. From 2011 to 2012, he was a Communications and Networks Engineer with Huawei Company. From 2014 to 2016, he was a Research Assistant with Qatar University, Doha, Qatar. His research interests are in the areas of wireless communications and networking, media streaming, heterogeneous wireless networks, compressive sensing with applications to communications, and signal processing for communications.
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./bio/vaneet.eps}}]{Vaneet Aggarwal (S'08 - M'11 - SM'15)}
	received the B.Tech. degree in 2005 from the Indian Institute of Technology, Kanpur, India, and the M.A. and Ph.D. degrees in 2007 and 2010, respectively from Princeton University, Princeton, NJ, USA, all in Electrical Engineering.
	
	He is currently an Assistant Professor at Purdue University, West Lafayette, IN. Prior to this, he was a Senior Member of Technical Staff Research at AT\&T Labs-Research, NJ, and an Adjunct Assistant Professor at Columbia University, NY. His research interests are in applications of statistical, algebraic, and optimization techniques to distributed storage systems, machine learning,  and wireless systems. Dr. Aggarwal was the recipient of Princeton University's Porter Ogden Jacobus Honorific Fellowship in 2009. He also received the 2017 Jack Neubauer Memorial Award recognizing the Best Systems Paper published in the {\em IEEE Transactions on Vehicular Technology}. He is serving on the editorial board of the {\em IEEE Transactions on Communications} and the {\em IEEE Transactions on Green Communications and Networking}. 
\end{IEEEbiography}

%\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./bio/tlan.eps}}]{Tian Lan (S'03-M'10)} received the B.A.Sc. degree from the Tsinghua University, China in 2003, the M.A.Sc. degree from the University of Toronto, Canada, in 2005, and the Ph.D. degree from the Princeton University in 2010. Dr. Lan is currently an Associate Professor of Electrical and Computer Engineering at the George Washington University. His research interests include cloud resource optimization, mobile networking, storage systems and cyber security. Dr. Lan received the 2008 IEEE Signal Processing Society Best Paper Award, the 2009 IEEE GLOBECOM Best Paper Award, and the 2012 INFOCOM Best Paper Award.
%\end{IEEEbiography}





%\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./bio/yu.eps}}]{Yu Xiang} received the B.A.Sc. degree from Harbin Institute of Technology in 2010, and the Ph.D. degree from George Washington University in 2015, both in Electrical Engineering. She is now a senior inventive scientist at AT\&T Labs-Research. Her current research interest are in cloud resource optimization, distributed storage systems and cloud storage charge-back.
%\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./bio/mooRyong}}]{Moo-Ryong Ra}
Moo-Ryong Ra joined AT\&T Labs Research in 2013 and is now working as a Principal Inventive Scientist in Cloud Platform Software Research department.  He is broadly interested in solving challenging problems related to cloud platforms, software-defined storage systems, and nowadays 5G RAN. His recent projects span across multiple areas-intelligent controller for 5G RAN, ultra low latency storage solutions with RDMA transport, storage-centric hardware/software design for AT\&T's Integrated Cloud and Edge Cloud, optimizing AT\&T,s video storage and delivery, data deduplication for distributed storage systems and enabling faster recovery of erasure-coded storage. He earned a PhD degree in the Computer Science Department at University of Southern California (USC). During his graduate study, he collaborated with other top-notch research labs such as Microsoft Research and Intel Labs in the area of mobile cloud computing. When opportunities arise, every now and then he teaches undergraduate/graduate courses in the ECE department at Rutgers University.
\end{IEEEbiography}

%\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./bio/robin.eps}}]{Yih-Farn (Robin) Chen}
%	is a Director of Inventive Science, leading the Cloud Platform Software Research department at AT\&T Labs  - Research.  His current research interests include cloud computing, software-defined storage, mobile computing, distributed systems, World Wide Web, and IPTV.  He holds a Ph.D. in Computer Science from University of California at Berkeley, an M.S. in Computer Science from University of Wisconsin, Madison,  and a B.S. in Electrical Engineering from National Taiwan University. Robin is an ACM Distinguished Scientist and a Vice Chair of the International World Wide Web Conferences Steering Committee (IW3C2).  He also serves on the editorial board of IEEE Internet Computing.
%\end{IEEEbiography}










==> dltimeWithEll.tex <==
\section{Download and Play Times of a Segment not Requested in $\omega_i$}


\label{sec:DownLoadPlay}

In order to characterize the stall duration tail probability, we need
to find the download time and the play time of different video segments, for any server $j$ and streams with the choice of $\beta_j$ and $\nu_j$, assuming file $i$ is not requested in the last  $\omega_i$ time-units and thus the file cannot be obtained from the edge-cache. The stochastic randomness in the choice of these variables will be considered in the overall metric. Further, the optimization over  decision variables will be considered in the optimization formulation. 

%In the following, we will first estimate the download time of segments from the cache servers and from datacenter, respectively. Then, based on the download time of each segment, we derive the play time of different segments and then give the stall duration expression for each segment request.

\subsection{Download Times of first $L_{j,i}$ Segments}

We consider a queuing model, where $W_{j,\nu_{j}}^{(e)}$ denotes the random  waiting time of all video files in the queue of $PS^{(e,j)}_{\nu_j}$ before file $i$ request is served, 
and $Y_{i,j,\nu_{j}}^{(e,g)}$ be the (random service time of a coded chunk
$g$ for file $i$ from server $j$ and queue $\nu_{j}$. Then, for $g\le L_{j,i}$, the random download time of the first $L_{j,i}$ segments $g\in\{1,\ldots,L_{j,i}\}$ if file $i$ is requested from stream $PS^{(e,j)}_{\nu_j,\ell}$,from edge-router $\ell$ is given as 
 \begin{equation}
D_{i,j,\beta_j,\nu_{j},\ell}^{(g)}=W_{j,\nu_{j},\ell}^{(e)}+\sum_{v=1}^{g}Y_{i,j,\nu_{j},\ell}^{(e,v)}
\end{equation}
Since video file $i$ consists of $L_{j,i}$ segments stored at cache
server $j$, the total service time for video file $i$ request from edge router $\ell$ at queue
$PS^{(e,j)}_{\nu_j,\ell}$, denoted by $ST_{i,j,\nu_{j},\ell}$, is given as 
\begin{equation}
ST_{i,j,\nu_{j},\ell}=\sum_{v=1}^{L_{j,i}}Y_{i,j,\nu_j,\ell}^{(e,v)}
\end{equation}
Hence, the service time of the video files at the parallel stream $PS^{(e,j)}_{\nu_j,\ell}$ is given as  
\begin{equation}
R_{j,\nu_{j},\ell}^{(e)}=\begin{cases}
ST_{i,j,\nu_{j},\ell}^{(e,L_{j,i})} \ \   \text { with prob. } \frac{\lambda_{i}\pi_{i,j,\ell}p_{i,j,\nu_j,\ell}e^{-\lambda_{i,\ell} \omega_{i,\ell}}}{\Lambda_{j,\nu_{j},\ell}^{(e)}}& \forall i\end{cases}
\end{equation}


We can show that the moment generating function of the service time for all video files from parallel stream $PS^{(e,j)}_{\nu_j,\ell}$   is given by 
\begin{align}
& B_{j,\nu_{j},\ell}^{(e)}(t)={\mathbb{E}}[e^{tR_{j,\nu_{j},\ell}^{(e)}}]\nonumber\\
& =\sum_{i=1}^{r}\frac{\lambda_{i,\ell}\pi_{i,j,\ell}p_{i,j,\nu_{j},\ell}e^{-\lambda_{i,\ell}\omega_{i,\ell}}}{\Lambda_{j,\nu_{j},\ell}^{(e)}}\left(\frac{\alpha_{j,\nu_{j},\ell}^{(e)}e^{\eta_{j,\nu_{j},\ell}^{(e)}t}}{\alpha_{j,\nu_{j},\ell}^{(e)}-t}\right)^{L_{j,i}}\label{Be}
\end{align}

Further, based on our 2-stage scheduling policy, the load intensity at $PS^{(e,j)}_{\nu_j,\ell}$  is as follows 
\begin{align}
\rho_{j,\nu_{j},\ell}^{(e)} & =\Lambda_{j,\nu_{j},\ell}^{(e)}B_{j,\nu_{j},\ell}^{(e)'}(0)\nonumber\\
& =\sum_{i=1}^{r}\lambda_{i,\ell}\pi_{i,j,\ell}p_{i,j,\nu_{j},\ell}e^{-\lambda_{i,\ell}\omega_{i,\ell}}L_{j,i}\left(\eta_{j,\nu_{j},\ell}^{(e)}+\frac{1}{\alpha_{j,\nu_{j},\ell}^{(e)}}\right)\label{rhoe}
\end{align}



Since the arrival is Poisson and the service time is shifted-exponentially distributed, the moment generating function (MGF) of the waiting time at queue $PS^{(e,j)}_{\nu_j}$ can be calculated usingthe  Pollaczek-Khinchine formula, i.e.,
%(since M/M/1 is a special case of M/G/1) 
%and is given by
\begin{align}
\mathbb{E}\left[e^{tW_{j,\nu_{j},\ell}^{(e)}}\right] & =\frac{(1-\rho_{j,\nu_{j},\ell}^{(e)})tB_{j,\nu_{j},\ell}^{(e)}(t)}{t-\Lambda_{j,\nu_{j},\ell}^{(e)}(B_{j,\nu_{j},\ell}^{(e)}(t)-1)}
\end{align}
From the MGF of $W_{j,\nu_{j},\ell}^{(e)}$ and the service
time, the MGF of the download time of segment $g$ from the queue $PS^{(e,j)}_{\nu_j}$ for file $i$ is then
\begin{equation}
\mathbb{E}\left[e^{tD_{i,j,\beta_j,\nu_{j},\ell}^{(g)}}\right]=\frac{(1-\rho_{j,\nu_{j},\ell}^{(e)})tB_{j,\nu_{j},\ell}^{(e)}(t)}{t-\Lambda_{j,\nu_{j},\ell}^{(e)}(B_{j,\nu_{j},\ell}^{(e)}(t)-1)}\left(\frac{\alpha_{j,\nu_{j},\ell}^{(e)}e^{\eta_{j,\nu_j,\ell}^{(e)}t}}{\alpha_{j,\nu_{j},\ell}^{(e)}-t}\right)^{g}
\label{D_nu_j}.
\end{equation}
We note that the above is defined only when MGFs exist, i.e., 
\begin{eqnarray}
t&<& \alpha_{j,\nu_{j},\ell}^{(e)}\label{alpha_j_nuj}\\
0 &<& t-\Lambda_{j,\nu_{j},\ell}^{(e)}(B_{j,\nu_{j},\ell}^{(e)}(t)-1)
\label{mgf_gz_e_queue}
\end{eqnarray}

%Finally, the overall download time of all the $L_{j,i}$ segments of video $i$ at the client,
%$D_{i}^{(g)}$ , is given by
%
%
%\begin{equation}
%D_{i}^{(g)}=\sum_{j=1}^{m}\pi_{i,j}\sum_{\nu_{j}=1}^{e_{j}}p_{j,\nu_{j}}D_{i,j,\nu_{j}}^{(g)},\,\,\,\,\,g\leq L_{j,i}
%\end{equation}




==> dltimelastWithell.tex <==
\subsection{Download Times of last $(L_i - L_{j,i})$ Segments }

\label{downloadtimelast}

Since the later video segments $(L_i - L_{j,i})$ are downloaded from the data center, we need to schedule them to the $\beta_j$ streams using the proposed probabilistic scheduling policy.
%and thus the choice is among the 
We first determine the time it takes for chunk $g$ to depart the first queue (i.e., $\beta_j$ queue at datacenter). For that, we define the time of chunk $g$ to depart the first queue as
\begin{equation}
E_{i,j,\beta_{j}}^{(g)}=W_{j,\beta_{j}}^{(d)}+\sum_{v=L_{j,i}+1}^{L_i}Y^{(d,v)}_{j,\beta_{j}},
\end{equation}
where $W_{j,\beta_{j}}^{(d)}$ is the waiting time from $PS^{(d,j)}_{\beta_j}$ for the earlier video segments, and $Y^{(d,v)}_{j,\beta_{j}}$ is the service time for obtaining segment $v$ from the queue of $PS^{(d,j)}_{\beta_j}$. Using similar analysis for that of deriving the MGF of download time of chunk $g$  as in the last section, we obtain
 \begin{equation}
 \mathbb{E}\left[e^{tE_{i,j,\beta_{j}}^{(g)}}\right]=\frac{(1-\rho_{j,\beta_{j}}^{(d)})tB_{j,\beta_{j}}^{(d)}(t)}{t-\Lambda^{(d)}_{j,\beta_{j}}(B_{j,\beta_{j}}^{(d)}(t)-1)}\left(\frac{\alpha_{j,\beta_{j}}^{(d)}e^{\eta_{j,\beta_j}^{(d)}t}}{\alpha_{j,\beta_{j}}^{(d)}-t}\right)^{g-L_{j,i}-1},
 \end{equation}
where the load intensity at queue $\beta_j$ at datacenter, $\rho_{j,\beta_{j}}^{(d)}$
\begin{align}
\rho_{j,\beta_{j}}^{(d)}= & \sum_{i=1}^{r}\lambda_{i}\pi_{i,j}q_{i,j,\beta_{j}}e^{-\lambda_{i}\omega_{i}}\left(L_{i}-L_{j,i}\right)\times\nonumber\\
& \left(\eta_{j,\beta_{j}}^{(\overline{d})}+\frac{1}{\alpha_{j,\beta_{j}}^{(d)}}\right)\label{rhoc}
\end{align}

\begin{align}
B_{j,\beta_{j}}^{(d)}(t) & =\sum_{i=1}^{r}\frac{\lambda_{i}\pi_{i,j}q_{i,j,\beta_{j}}e^{-\lambda_{i}\omega_{i}}}{\Lambda_{j,\beta_{j}}^{(c)}}\left(\frac{\alpha_{j,\beta_{j}}^{(d)}e^{\eta_{j,\beta_{j}}^{(d)}t}}{\alpha_{j,\beta_{j}}^{(d)}-t}\right)^{L_{i}-L_{j,i}}\label{Bc}
\end{align}
% $\rho_{j,\beta_{j}}^{(d)} = ??$ and $B_{j,\beta_{j}}^{(d)}(t) = ??$.
 
%{\color{blue} Add a couple of sentences here to explain why it can be derived recursively.} 
To find the download time of video segments from the second queue (at cache server $j$), we notice that the download time for segment $g$ includes the waiting to download all previous segments and the idle time if the segment $g$ is not yet downloaded from the first queue ($PS^{(d,j)}_{\beta_j}$), as well as the service time of the segment from $PS^{(\overline{d},j)}_{\beta_j}$. Then, the download time of the video segments from the second queue (i.e.,$PS^{(\overline{d},j)}_{\beta_j,\ell}$) can be derived by a set of recursive equations, with download time of the first (initial) segment $(L_{j,i}+1)$ as 
 \begin{equation}
D_{i,j,\beta_{j},\nu_j,\ell}^{(L_{j,i}+1)} = \max(W_{j,\beta_{j},\ell}^{(\overline{d})},  E_{j,\beta_{j}}^{(L_{j,i}+1)}) + Y^{(\overline{d},L_{j,i}+1)}_{j,\beta_{j},\ell},
 \end{equation}
where $W_{j,\beta_{j},\ell}^{(\overline{d})}$ is the waiting time from queue $PS^{(\overline{d},j)}_{\beta_j,\ell}$ for the previous video segments, and $Y^{(\overline{d},v)}_{j,\beta_{j},\ell}$ is the required service time for obtaining segment $v$ from the queue of $PS^{(\overline{d},j)}_{\beta_j,\ell}$. The download time of the following segments ($g>L_{j,i}+1$) is given by the following recursive equation 
\begin{equation}
D_{i,j,\beta_{j},\nu_j,\ell}^{(g)} = \max(D_{i,j,\beta_{j},\nu_j,\ell}^{(g-1)},  E_{i,j,\beta_{j}}^{(g)}) + Y^{(\overline{d},g)}_{j,\beta_{j},\ell}.
\end{equation}
%This is because the download time for segment $g$ has to 

With the above recursive equations from $y=L_{j,i}$ to $y=g$, we can obtain that 
\begin{equation}
D_{i,j,\beta_{j},\nu_j,\ell}^{(g)} = \max_{y=L_{j,i}}^g U_{i,j,\beta_j,g,y,\ell},
\end{equation}
where
\begin{equation}
U_{i,j,\beta_j,g,L_{j,i},\ell} = W_{j,\beta_{j},\ell}^{(\overline{d})} + \sum_{h= L_{j,i}+1}^gY^{(\overline{d},h)}_{j,\beta_{j},\ell}
\end{equation}
Similarly, for $y>L_{j,i}$, we have
\begin{equation}
U_{i,j,\beta_j,g,y,\ell} = E_{i,j,\beta_{j}}^{(y)} + \sum_{h= y}^gY^{(\overline{d},h)}_{j,\beta_{j},\ell}.
\end{equation}

It is easy to see that the moment generating function of $U_{i,j,\beta_j,g,y,\ell}$ for $y=L_{j,i}$ is given by
\begin{equation}
\mathbb{E}[e^{tU_{i,j,\beta_{j},g,L_{j,i}},\ell}]=  \!\!\frac{(1-\rho_{j,\beta_{j},\ell}^{(\overline{d})})tB_{j,\beta_{j},\ell}^{(\overline{d})}(t)}{t-\Lambda_{j,\beta_{j}}^{(c)}(B_{j,\beta_{j},\ell}^{(\overline{d})}(t)-1)}\!\!\left(\!\!\!\frac{\alpha_{j,\beta_{j},\ell}^{(\overline{d})}e^{\eta_{j,\beta_{j},\ell}^{(\overline{d})}t}}{\alpha_{j,\beta_{j},\ell}^{(\overline{d})}-t}\!\!\right)^{g-L_{j,i}},
\label{U_MGF_Lji}
\end{equation}
where the load intensity at queue $\beta_j$ at cache server $j$, $\rho_{j,\beta_{j}}^{(\overline{d})}$ is given by 
%\begin{align}
%\rho_{j,\beta_{j}}^{(\overline{d})} & =\sum_{i=1}^{r}\lambda_{i}\pi_{i,j}q_{i,j,\beta_j}e^{-\lambda_i \omega_i}\left( L_i-L_{j,i}\right)\left( \eta_{j,\beta_j}^{(\overline{d})}+ \frac{1}{\alpha_{j,\beta_{j}}^{(\overline{d})}}\right)\label{rhoc}\\
%B_{j,\beta_{j}}^{(\overline{d})}(t) & =\sum_{i=1}^{r}\frac{\lambda_{i}\pi_{i,j}q_{i,j,\beta_j}e^{-\lambda_i \omega_i}}{\Lambda_{j,\beta_{j}}^{(c)}}\left(\frac{\alpha_{j,\beta_{j}}^{(\overline{d})}e^{\eta_{j,\beta_j}^{(\overline{d})}t}}{\alpha_{j,\beta_{j}}^{(\overline{d})}-t}\right)^{L_{i}-L_{j,i}}\label{Bc}
%\end{align}
\begin{align}
\rho_{j,\beta_{j},\ell}^{(\overline{d})}= & \sum_{i=1}^{r}\lambda_{i,\ell}\pi_{i,j,\ell}q_{i,j,\beta_{j},\ell}e^{-\lambda_{i,\ell}\omega_{i,\ell}}\left(L_{i}-L_{j,i}\right)\times\nonumber\\
& \left(\eta_{j,\beta_{j},\ell}^{(\overline{d})}+\frac{1}{\alpha_{j,\beta_{j},\ell}^{(\overline{d})}}\right)\label{rhoc}\\
B_{j,\beta_{j},\ell}^{(\overline{d})}(t) & =\sum_{i=1}^{r}\frac{\lambda_{i,\ell}\pi_{i,j,\ell}q_{i,j,\beta_{j,\ell}}e^{-\lambda_{i,\ell}\omega_{i,\ell}}}{\Lambda_{j,\beta_{j},\ell}^{(\overline{d})}}\left(\frac{\alpha_{j,\beta_{j},\ell}^{(\overline{d})}e^{\eta_{j,\beta_{j},\ell}^{(\overline{d})}t}}{\alpha_{j,\beta_{j},\ell}^{(\overline{d})}-t}\right)^{L_{i}-L_{j,i}}\label{Bc}
\end{align}
Similarly, the moment generating function of $U_{i,j,\beta_j,g,y}$ for $y>L_{j,i}$ is given as 
\begin{align}
\mathbb{E}[e^{tU_{i,j,\beta_{j},g,y,\ell}}] & =\overline{W}_{j,\beta_{j}}^{(d)}\times \nonumber\\
& \left(\frac{\alpha_{j,\beta_{j}}^{(d)}e^{\eta_{j,\beta_{j}}^{(d)}t}}{\alpha_{j,\beta_{j}}^{(d)}-t}\right)^{y-L_{j,i}-1}\left(\frac{\alpha_{j,\beta_{j}}^{(\overline{d})}e^{\eta_{j,\beta_{j}}^{(\overline{d})}t}}{\alpha_{j,\beta_{j}}^{(\overline{d})}-t}\right)^{g-y+1}
\label{U_MGF_all}
\end{align}
%{\mathbb E}[e^{tU_{i,j,\beta_j,g,y}}] = \frac{(1-\rho_{j,\beta_{j}}^{(d)})tB_{j,\beta_{j}}^{(d)}(t)}{t-\Lambda^{(d)}_{j,\beta_{j}}(B_{j,\beta_{j}}^{(d)}(t)-1)}\left(\frac{\alpha_{j,\beta_{j}}^{(d)}}{\alpha_{j,\beta_{j}}^{(d)}-t}\right)^{y-L_{j,i}-1}\left(\frac{\alpha_{j,\beta_{j}}^{(c)}}{\alpha_{j,\beta_{j}}^{(c)}-t}\right)^{g-y+1}.
where $\overline{W}_{j,\beta_{j}}^{(d)}=\frac{(1-\rho_{j,\beta_{j}}^{(d)})tB_{j,\beta_{j}}^{(d)}(t)}{t-\Lambda_{j,\beta_{j}}^{(d)}(B_{j,\beta_{j}}^{(d)}(t)-1)}$.
We further note that these moment generating functions are only defined when the MGF functions exist, i.e., 
%\begin{eqnarray}
%t&<& \alpha_{j,\beta_{j}}^{(d)}\label{alpha_betaj_d}\\
%0 &<& t-\Lambda_{j,\beta_{j}}^{(d)}(B_{j,\beta_{j}}^{(d)}(t)-1)\\
%t&<& \alpha_{j,\beta_{j}}^{(\overline{d})}\\
%0 &<& t-\Lambda_{j,\beta_{j}}^{(\overline{d})}(B_{j,\beta_{j}}^{(\overline{d})}(t)-1)
%\label{mgf_beta_j_c}
%\end{eqnarray}
\begin{eqnarray}
t<\alpha_{j,\beta_{j}}^{(d)}\label{alpha_betaj_d};\,\,\,\,
0 < t-\Lambda_{j,\beta_{j}}^{(d)}(B_{j,\beta_{j}}^{(d)}(t)-1)\\
t< \alpha_{j,\beta_{j}}^{(\overline{d})};\,\,\,\,
0 < t-\Lambda_{j,\beta_{j},\ell}^{(\overline{d})}(B_{j,\beta_{j},\ell}^{(\overline{d})}(t)-1)
\label{mgf_beta_j_c}
\end{eqnarray}





==> downLoadPlayTimeMain.tex <==





\section{Download and Play Times of a Segment not Requested in $\omega_i$}

Here, we need to talk about Download time and play time of the chunks

\subsection{Download Times of first $L_{j,i}$ Segments}



\subsection{Download Times of last $(L_i - L_{j,i})$ Segments }


\subsection{Play Times of different Segments}

==> dwnloadPlyTime.tex <==
\input{dltime}
\input{dltimelast}
\input{pltime}

==> online.tex <==

\subsection{Online Algorithm for Edge-cache Placement}\label{sec:adapt}

We note that for the setup of the edge cache, we assumed that the edge-cache has a capacity of $C_{e}$ seconds (ignoring the index of the edge cache). However, in the caching policy, we assumed that a file $i$ is removed from the cache if it has not been requested in the last $\omega_i$ seconds. In the optimization, we found the parameters $\omega_i$, such that the cache capacity is exceeded with probability less than $\epsilon$. However, this still assumes that it is possible to exceed the cache capacity some times. This is, in practice, not possible. Thus, we will propose a mechanism to adapt the decision obtained by the optimization formulation so as to never exceed the edge cache capacity. 

When a file $i$ is requested, the last request of file $i$ is first checked. If it has not been requested in the last $\omega_i$ seconds, it is obtained from the CDN. In order to do that, the space of the file is reserved in the edge-cache. If this reservation exceeds the capacity of the edge-cache, certain files have to be removed. Any file $f$ that has not been requested in the last $\omega_f$ seconds is removed from the cache. If, even after removing these files, the space in the edge-cache is not enough for placing file $i$ in the edge-cache, more files must be removed. Assume that  $\mathcal{H}$ is the set contains all files in the edge-cache, and $t_{f,\ell}$ is the last time file $f$ has been requested. Then, if another file needs to be removed to make space for the newly requested file, the file $\underset{j\in\mathcal{H}}{\arg \min}\,(t_{k,\ell}+\omega_{k}-t_{i})$ is removed. This continues till there is enough space for the new incoming file. Note that multiple files may have to be removed to make space for the incoming file, depending on the length of the new file. This is similar in concept to LRU where a complete new file is added in the cache, and multiple small files may have to be removed to make space. The key part of the online adaptation so as not to violate the edge-cache capacity constraint is illustrated in Figure \ref{fig:flowchart}.

{\bf Abubakr, adapt the flowchart based on the explanations above. Also, some mention of schematic should be there - it is not clear how to read that figure. Also, you only have $t_i$ - $t_1$, etc. in figure are not consistent - remove the figure or explain better. }
% If it is previously requested within a period of $\omega_i$, then the file is locally stored and, hence, directly served from the edge-cache. If not, request for file $i$ is sent to the top caching levels and then placed into the edge-cache after being served. If the edge-cache is full, the video file that its window is about to expire is removed, i.e., $\underset{j\in\mathcal{H}}{\text{min}}\,(t_{j,\ell}+\omega_{j}-t_{i})$, where $j\ne i$, $t_{j,\ell}$ is the last request for file $j$, and $\mathcal{H}$ is the set contains all files in the edge-cache, and then the new requested file $i$ is placed instead. These details are summarized in Figure \ref{fig:flowchart}.




%For the algorithm described in the previous section, we assumed
%that the file placement on the edge-cache is fixed. However, in practice, the content in the cache can change due to the variations on the patten of the video file requests. Hence, in this section, we propose an online version of our algorithm to capture the system's dynamics of adding and/or ejecting the video files from the edge-cache. We note that the edge-cache capacity at the edge-router is limited, and thus can store up to $C_{j,e}$ seconds at most. Therefore, if the edge-cache is full and a request for a non-cached video file (not already stored in the cache) is arrived at the edge-router, one file has to be removed before adding the new requested video file. Thus, to make a space for a new video file, the file that its window-size $\omega_i$ is about to expire is evicted. This eviction policy is aligned with that of the well-know Least-Recently-Used (LRU) policy except that we look back only to $\omega_i$ units of time rather than the whole previous past time. While the algorithm parameters are optimized offline, our results show that the online algorithm still performs very close to the offline algorithm as only few video files need to be inserted into the cache over a relatively large window size. As a result, one can run the offline algorithm at a certain rate, i.e., one every a few hours, and then use the optimized parameters to run the online algorithm. The rate of running the offline optimization algorithm depends on factors like the rate of change in the pattern of video file requests, overhead that the system can handle, traffic at the origin server, ...etc. We note that while Constraint \eqref{P_N_j} probabilistically bounding the content in edge-cache to be less than $N_{t}$, we relaxed that constraint in our implementation for the online algorithm to (deterministically) force the number of files to be exactly $N_t$. As will be shown in our extensive experimental results, this constraint is only an upper-bound and the actual probability turns out to be much less than this value. 

 
\begin{figure}[t]
	\centering
	\includegraphics[trim=00.0in 0.00in 0.00in 0.00in, clip, width=0.47\textwidth]{onlineFlowChart/flowchart}
	%	\vspace{-.45in}
	\caption{\small A flowchart illustrates the online updates for an edge-cache when a file $i$ is requested at time $t_i$. Here, $t_{j,\ell}$ represents the time of the last request of file $i$ from edge-cache $j$, and $\mathcal{H}$ is the index set of all video files in the edge-cache. \label{fig:flowchart}}
	%	\vspace{-.25in}
\end{figure}

\begin{figure}[t]
	\centering
	\includegraphics[trim=00.0in 0.00in 0.00in 0.00in, clip, width=0.47\textwidth]{onlineFlowChart/windowsize}
	%	\vspace{-.45in}
	\caption{\small A schematic showing an example of how a time-line of a file $i$ can change over the time.
		 \label{fig:windowSize}}
	%	\vspace{-.25in}
\end{figure}


%In the , we present our evaluation results for our proposed scheme considering both offline and online versions of our proposed algorithm. 


==> p_opt.tex <==
\subsubsection{PS Selection Probabilities}
Given the auxiliary variables, the bandwidth allocation weights, the streamed video quality probabilities, and the scheduling probabilities, this subproblem can be written as follows. 

\textbf{Input: $\boldsymbol{q}$, $\boldsymbol{b}$, $\boldsymbol{t}$, and $\boldsymbol{w}$}

\textbf{Objective:} $\qquad\quad\;\;$min $\left(\ref{eq:joint_otp_prob}\right)$

$\hphantom{\boldsymbol{\text{Objective:}\,}}\qquad\qquad$s.t. 
\eqref{eq:rho_j},
\eqref{eq:Lambda_j},
\eqref{eq:sum_p_nuj},
\eqref{eq:don_pos_cond2},

$\hphantom{\boldsymbol{\text{Objective:}\,}}\qquad\qquad$var. $\boldsymbol{p}$

 This optimization can be solved using NOVA algorithm. The constraints  \eqref{eq:rho_j}, \eqref{eq:Lambda_j}, \eqref{eq:sum_p_nuj}, and \eqref{eq:don_pos_cond2} are linear in $\boldsymbol{p}$, and hence, the domain is convex. 

 Algorithm \ref{alg:NOVA_Alg5} (given in Appendix \ref{apdx_table}) shows the used procedure to solve for $\boldsymbol{p}$. Let ${U_p}\left(\boldsymbol{p};\boldsymbol{p^\nu}\right)$ be the
convex approximation at iterate $\boldsymbol{p^\nu}$ to the original non-convex problem $U\left(\boldsymbol{p}\right)$, where $U\left(\boldsymbol{p}\right)$ is given by (\ref{eq:joint_otp_prob}), assuming other parameters constant. Then, a valid choice of  ${U_p}\left(\boldsymbol{p};\boldsymbol{p^\nu}\right)$ is the first order approximation of  $U\left(\boldsymbol{p}\right)$, i.e.,  
\begin{equation}
{U_p}\left(\boldsymbol{p},\boldsymbol{p^\nu}\right)=\nabla_{\boldsymbol{p}}U\left(\boldsymbol{p^\nu}\right)^{T}\left(\boldsymbol{p}-\boldsymbol{p^\nu}\right)+\frac{\tau_{p}}{2}\left\Vert \boldsymbol{p}-\boldsymbol{b^\nu}\right\Vert ^{2}.\label{eq:U_b}
\end{equation}
where $\tau_p$ is a regularization parameter. The detailed steps can be seen in Algorithm \ref{alg:NOVA_Alg5}. Since all the constraints  have been shown to be convex in $\boldsymbol{p}$, the optimization problem in Step 1 of  Algorithm \ref{alg:NOVA_Alg5} can be solved by the standard projected gradient descent algorithm. 

%Similar to Access  Optimization problem, we get the minimizer for (\ref{eq:U_t_u_bar}), step 1 in Algorithm \ref{alg:NOVA_Alg1}), and then continue until convergence. 


%In this sub-problem, we solve for all $t_i$, for fixed placement and given accessing probabilities. Similar to $\boldsymbol{\pi}$- Optimization problem, we used NOVA algorithm to solve for $t$.  Algorithm \ref{alg:NOVA_Alg1}, shows the used procedure to solve for $\boldsymbol{t}$. After initialization with feasible choice, NOVA keeps generating  a sequence of monotonically decreasing $\left\{ \boldsymbol{t}^{\nu+1}\right\} $ until  convergence.



\begin{lemma} \label{lem_t}

For fixed $\boldsymbol{t}$, $\boldsymbol{w}$, $\boldsymbol{b}$, and  $\boldsymbol{q}$, the optimization of our problem over 
$\boldsymbol{p}$ generates a sequence of monotonically decreasing
objective values and therefore is guaranteed to converge to a stationary point.
\end{lemma}
%\begin{proof}
%Since NOVA Algorithm generates a sequence of monotonically decreasing
%objective values as shown in \cite{scutNOVA}, $\boldsymbol{t}$ is guaranteed to converge to a stationary point.
%\end{proof}




==> pltimeWithell.tex <==
\subsection{Play Times of different Segments}

Next, we find the play time of different video segments. Recall that $D_{i,j,\beta_{j},\nu_{j},\ell}^{(g)}$ is the download time of segment
$g$ from $\nu_{j}$ from edge router $\ell$ and $\beta_{j}$ queues at client $i$. We further define $T_{i,j,\beta_j,\nu_j,\ell}^{\left(g\right)}$ as the time that segment $g$ begins to play at the client $i$, given that it is downloaded from $\beta_j$ and $\nu_j$ queues requested through edge router $\ell$. This start-up delay of the video is denoted by $d_{s}$. Then, the first segment is ready for play at the maximum
of the startup delay and the time that the first segment can be downloaded. This means
\begin{equation}
T_{i,j,\beta_j,\nu_j,\ell}^{(1)}=\mbox{max }\left(d_{s},\,D_{i,j,\beta_j,\nu_j,\ell}^{(1)}\right).
\end{equation}


For $1<g\le L_{i}$, the play time of segment $g$ of video file $i$ is
given by the maximum of (i) the time to download the segment
and (ii) the time to play all previous segment plus the time
to play segment $g$ (i.e., $\tau$ seconds). Thus, the play time of segment
$g$ of video file $i$, when requested from server, $j$ edge router $\ell$, and from $\nu_j$ and $\beta_j$ queues, can be expressed as 
%$T_{i,j,\beta_j,\nu_j}^{(q)}$
\begin{equation}
T_{i,j,\beta_j,\nu_j,\ell}^{(q)}=\mbox{max }\left(T_{i,j,\beta_j,\nu_j,\ell}^{(q-1)}+\tau,\,D_{i,j,\beta_j,\nu_j}^{(q)}\right).\label{eq:T_ij_general}
\end{equation}
%Equation (\ref{eq:T_ij_general}) 
This results in a set of recursive equations, which further yield by
\begin{align}
T_{i,j,\beta_{j},\nu_{j},\ell}^{(L_{i})} & =\mbox{max }\left(T_{i,j,\beta_{j},\nu_{j},\ell}^{(L_{i}-1)}+\tau,\,D_{i,j,\beta_{j},\nu_{j},\ell}^{(L_{i})}\right)\nonumber \\
 & =\mbox{max }\left(T_{i,j,\beta_{j},\nu_{j},\ell}^{(L_{i}-2)}+2\tau,\,D_{i,j,\beta_{j},\nu_{j},\ell}^{(L_{i}-1)}+\tau,\,D_{i,j,\beta_{j},\nu_{j},\ell}^{(L_{i})}\right)\nonumber \\
 & =\!\mbox{max}\left(d_{s}+(L_{i}-1)\tau,\,\max_{z=2}^{L_{i}+1}D_{i,j,\beta_{j},\nu_{j},\ell}^{(z-1)}+(L_{i}-z+1)\tau\right)\nonumber \\
 & =\overset{L_{i}+1}{\underset{z=1}{\text{max}}}\,\mathcal{F}_{i,j,\beta_{j},\nu_{j},\ell,z}
 \label{T_ijbetanuF}
\end{align}
where $\mathcal{F}_{i,j,\beta_{j},\nu_{j},\ell,z}$ is expressed as
\begin{equation}
\mathcal{F}_{i,j,\beta_{j},\nu_{j},\ell,z}=\begin{cases}
d_{s}+(L_{i}-1)\tau & \,,z=1\\
D_{i,j,\beta_{j},\nu_{j},\ell}^{(z-1)}+(L_{i}-z+1)\tau & 1<z\leq L_{i}
\end{cases} \label{F_1}
\end{equation}

We now get the MGFs of the 
$\mathcal{F}_{i,j,\nu_{j},\beta_{j},\ell,z}$ to use in characterizing the play time of the different segments. Towards this goal, we plug Equation (\ref{F_1}) into $\mathbb{E}\left[e^{t\mathcal{F}_{i,j,\nu_{j},\beta_{j},\ell,z}}\right]$ and obtain
%can be calculated as follows
%\begin{equation}
%\mathbb{E}\left[e^{t\mathcal{F}_{i,j,\nu_{j},\beta_{j},z}}\right]=\begin{cases}
%e^{(d_{s}+(L_{i}-1)\tau)t} & \,,z=1\\
%e^{(L_{i}-z+1)\tau t}\mathbb{E}\left[e^{tD_{i,j,\beta_{j},\nu_{j}}^{(z-1)}}\right] & 1<z\leq (L_{i}+1)
%\end{cases}
%\label{MGF_F}
%\end{equation}
\begin{align}
& \mathbb{E}\left[e^{t\mathcal{F}_{i,j,\nu_{j},\beta_{j},\ell,z}}\right]=\nonumber \\
\hphantom{} & \begin{cases}
e^{(d_{s}+(L_{i}-1)\tau)t} & \,,z=1\\
e^{(L_{i}-z+1)\tau t}\mathbb{E}\left[e^{tD_{i,j,\beta_{j},\nu_{j},\ell}^{(z-1)}}\right] & 1<z\leq(L_{i}+1)
\end{cases}\label{MGF_{F}}
\end{align}
where $\mathbb{E}\left[e^{tD_{i,j,\beta_{j},\nu_{j},\ell}^{(z-1)}}\right]$ can be calculated using equation (\ref{D_nu_j}) when $1<z\leq (L_{j,i}+1)$ and using equation (\ref{U_MGF_all}) when $z>L_{j,i}+1$ .
%
%where $Z_{D_{i,j,\nu_{j}}^{(z-1)}}$ is given by (\ref{D_nu_j}) and $Z_{D_{i,j,\beta_{j},\nu_j}^{(z-1)}}$ is given as follows.
%
%\begin{align}
%Z_{D_{i,j,\beta_{j},\nu_{j}}^{(z-1)}} & =\mathbb{E}\left[e^{tD_{i,j,\beta_{j},\nu_{j}}^{(z-1)}}\right]=\mathbb{E}\left[e^{t(\underset{y}{\text{\ensuremath{\max}}}U_{i,j,\beta_{j},g,y})}\right]\\
% & =\mathbb{E}\left[\underset{y}{\text{\ensuremath{\max}}}\,\,e^{tU_{i,j,\beta_{j},g,y}}\right]\\
% & \leq\sum_{y}e^{tU_{i,j,\beta_{j},g,y}}\\
% & =\left[e^{tU_{i,j,\beta_{j},g,L_{j,i}}}\right]+\sum_{w=L_{j,i}+1}^{g}\frac{(1-\rho_{j,\beta_{j}}^{(d)})tB_{j,\beta_{j}}^{(d)}(t)}{t-\Lambda_{j,\beta_{j}}^{(d)}(B_{j,\beta_{j}}^{(d)}(t)-1)}\left(\frac{\alpha_{j,\beta_{j}}^{(d)}}{\alpha_{j,\beta_{j}}^{(d)}-t}\right)^{w-L_{j,i}-1}\left(\frac{\alpha_{j,\beta_{j}}^{(c)}}{\alpha_{j,\beta_{j}}^{(c)}-t}\right)^{g-w+1}.
% \label{MGF_Z_D_last}
%\end{align}
%where $\left[e^{tU_{i,j,\beta_{j},g,L_{j,i}}}\right]$ is given in (\ref{U_MGF_Lji}).
The last segment should be completed by time $d_{s}+L_{i}\tau$ (which is the time at which the playing of the $L_i-1$ segment finishes). Thus, 
the difference between the play time of the last segment $T_{i,j,\beta_{j},\nu_{j},\ell}^{(L_{i})}$ and
$d_{s}+\left(L_{i}-1\right)\tau$ gives the stall duration. We note that
the stalls may occur before any segment and hence this difference will give
the sum of durations of all the stall periods before any segment. Thus, the stall duration for the request of file $i$ from $\beta_{j}$ queue,  $\nu_{j}$ queue and server $j$, edge router $\ell$ i.e., $\Gamma^{(i,j,\beta_{j},\nu_{j},\ell)}_{U}$ is given as
\begin{equation}
\Gamma^{(i,j,\beta_{j},\nu_{j},\ell)}_{U}=T_{i,j,\beta_{j},\nu_{j},\ell}^{(L_{i})}-d_{s}-\left(L_{i}-1\right)\tau 
\label{stallTimeap}
\end{equation}
%Next, we use this expression to derive a tight bound on the SDTP. 

==> probForm_SolApp.tex <==
%\section{Optimization Problem Formulation and Proposed Algorithm }
%\label{sec:SDTP}
%\subsection{Problem Formulation}
%We define 
%%$\boldsymbol{\pi}=(\pi_{i,j}\forall i=1,\cdots,r\text{ and }j=1,\cdots,m)$,
%%$\boldsymbol{p}=(p_{i,,j,\nu_{j}}\forall i=1,\cdots,r\,,j=1,\cdots,m\,,\,\nu_{j}=1,\ldots e_{j}),$
%%$\boldsymbol{q}=(q_{i,,j,\beta_{j}}\forall i=1,\cdots,r\,,j=1,\cdots,m\,,\,\beta_{j}=1,\ldots d_{j}),$ $\boldsymbol{t}=\left(t_{1},t_{2},\ldots,t_{r}\right)$, 
%%
%%$\boldsymbol{w}_{j,\beta_{j}}^{(c)}=(w_{j,1}^{(c)},w_{j,2}^{(c)},\ldots,w_{j,d_{j}}^{(c)},\text{ and }j=1,\cdots,m)$,
%%$\boldsymbol{w}_{j,\beta_{j}}^{(e)}=(w_{j,1}^{(e)},w_{j,2}^{(e)},\ldots,w_{j,d_{j}}^{(e)},\text{ and }j=1,\cdots,m)$,
%%$\boldsymbol{w}_{j,\beta_{j}}^{(d)}=(w_{j,1}^{(d)},w_{j,2}^{(d)},\ldots,w_{j,d_{j}}^{(d)},\text{ and }j=1,\cdots,m)$,
%%$\boldsymbol{L}_{j,i}=(L_{j,i},\,\forall i,\,\forall j)$
%
%$\ensuremath{\boldsymbol{\pi}=(\pi_{i,j}\forall i=1,\cdots,r\text{ and }j=1,\cdots,m)},$, $\boldsymbol{p}=(p_{i,,j,\nu_{j}}\forall i=1,\cdots,r\,,j=1,\cdots,m\,,\,\nu_{j}=1,\ldots e_{j})$, $\ensuremath{\boldsymbol{q}=(q_{i,,j,\beta_{j}}\forall i=1,\cdots,r\,,j=1,\cdots,m\,,\,\beta_{j}=1,\ldots d_{j}),}$, $\boldsymbol{h}=\left(h_{1},t_{2},\ldots,h_{r}\right)\,$, 
%$\ensuremath{\boldsymbol{w}^{(\overline{d})}=(w_{j,1}^{(\overline{d})},\ldots,w_{j,d_{j}}^{(c)}$,$\text{ and }j=1,\cdots,m)}\,,$, $\boldsymbol{w}^{(e)}=(w_{j,1}^{(e)},w_{j,2}^{(e)},\ldots,w_{j,d_{j}}^{(e)},\text{ and }j=1,\cdots,m)\,$ $\ensuremath{\boldsymbol{w}^{(d)}=(w_{j,1}^{(d)},\ldots,w_{j,d_{j}}^{(d)},\text{ and }j=1,\cdots,m)},$, $\boldsymbol{L}=(L_{j,i},\,\forall i=1,\,\text{ and }j=1,\cdots,m)$ and $\boldsymbol{\omega}=(\omega_i, \forall i)$.
%Our goal is to minimize the SDTP  over the
%choice of cache and datacenter access decisions, bandwidth allocation
%weights, portion (number) of cached segments, time window over which we maintain the video files at edge-cache and auxiliary bound parameters.
%
%To incorporate for weighted fairness and differentiated services,
%we assign a positive weight $\varpi_{i}$ for each file $i$. Without
%loss of generality, each file $i$ is weighted by the arrival rate
%$\lambda_{i}$ in the objective (so larger arrival rates are weighted
%higher). However, any other weights can be incorporated to accommodate
%for weighted fairness or differentiated services. Let $\overline{\lambda}=\sum_{i}\lambda_{i}$
%be the total arrival rate. Hence, $\varpi_{i}=\lambda_{i}/\overline{\lambda}$
%is the ratio of file $i$ requests. Hence, the objective is the minimization
%of stall duration tail probability, averaged over all the file requests,
%and is given as $\sum_{i}\frac{\lambda_{i}}{\overline{\lambda}}\,\text{\text{Pr}}\left(\Gamma^{(i)}\geq\sigma\right)$.
%By using the expression for SDTP in Section \ref{sec:StallTailProb},
%the optimization problem can be formulated as follows.
%
%%\begin{align}
%%%\text{\textbf{min}\,\,\,\,\,}\sum_{i=1}^{r}\frac{\lambda_{i}}{\overline{\lambda}} & \sum_{j=1}^{m}\pi_{i,j}\left[e^{-t_{i}\sigma}+\sum_{\nu_{j}=1}^{e_{j}}p_{i,j,\nu_{j}}e^{(\widetilde{\sigma}-\overline{\sigma})t_{i}}\frac{M_{j,\nu_{j}}^{(e)}(t_i)(1-\rho_{j,\nu_{j}}^{(e)})t_iB_{j,\nu_{j}}^{(e)}(t_i)}{t_i-\Lambda_{j,\nu_{j}}^{(e)}(B_{j,\nu_{j}}^{(e)}(t_i)-1)}\frac{\left((M_{j,\nu_{j}}^{(e)}(t_i))^{L_{j,i}}-1\right)}{M_{j,\nu_{j}}^{(e)}(t_i)-1}\right. \nonumber \\
%%%& +\sum_{\beta_{j}=1}^{d_{j}}q_{i,j,\beta_{j}}e^{(\widetilde{\sigma}-\overline{\sigma})t_{i}}\frac{(1-\rho_{j,\beta_{j}}^{(c)})t_iB_{j,\beta_{j}}^{(c)}(t_i)}{t_i-\Lambda_{j,\beta_{j}}^{(c)}(B_{j,\beta_{j}}^{(c)}(t_i)-1)}\left(\frac{\alpha_{j,\beta_{j}}^{(c)}}{\alpha_{j,\beta_{j}}^{(c)}-t_i}\right)^{L_{i}-L_{j,i}} (L_i - L_{j,i})\nonumber \\
%%%& +  \sum_{\beta_{j}=1}^{d_{j}}q_{i,j,\beta_{j}}e^{(\widetilde{\sigma}-\overline{\sigma})t_{i}}\frac{(1-\rho_{j,\beta_{j}}^{(d)})t_iB_{j,\beta_{j}}^{(d)}(t_i) \left(\widetilde{M}_{j,\beta_{j}}^{(d,c)}(t_i)\right)^{L_{j,i}+1}}{t_i-\Lambda_{j,\beta_{j}}^{(d)}(B_{j,\beta_{j}}^{(d)}(t_i)-1)}\left(\frac{\alpha_{j,\beta_{j}}^{(d)}-t_i}{\alpha_{j,\beta_{j}}^{(d)}}\right)^{L_{j,i}+1}\left(\frac{\alpha_{j,\beta_{j}}^{(c)}}{\alpha_{j,\beta_{j}}^{(c)}-t_i}\right)^{L_{i}+1} \nonumber\\
%%%& \left.  \left(\frac{\left(\widetilde{M}_{j,\beta_{j}}^{(d,c)}(t_i)\right)^{L_i-L_{j,i}}-(L_i-L_{j,i})}{\widetilde{M}_{j,\beta_{j}}^{(d,c)}(t_i)-1}+ \frac{\widetilde{M}_{j,\beta_{j}}^{(d,c)}(t_i)\left(\left(\widetilde{M}_{j,\beta_{j}}^{(d,c)}(t_i)\right)^{L_i-L_{j,i}-1}-1\right)}{\left(\widetilde{M}_{j,\beta_{j}}^{(d,c)}(t_i)-1\right)^2}\right)\right]label\label{eq:optfun}\\
%%%\boldsymbol{\text{s.t.}}\nonumber \\
%%% & \Lambda_{j,\beta_{j}}^{(d)}=\sum_{i=1}^{r}\lambda_{i}\pi_{i,j}q_{i,j,\beta_{j}},\,\,\,\forall j,\beta_{j}\label{eq:Lamda_d}\\
%%% & \Lambda_{j,\beta_{j}}^{(c)}=\sum_{i=1}^{r}\lambda_{i}\pi_{i,j}q_{i,j,\beta_{j}},\,\,\,\forall j,\beta_{j}\label{eq:Lamda_c}\\
%%% & \Lambda_{j,\nu_{j}}^{(e)}=\sum_{i=1}^{r}\lambda_{i}\pi_{i,j}p_{i,j,\nu_{j}},\,\,\,\forall j,\nu_{j}\label{eq:Lamda_e}\\
%%% & M_{j,\nu_{j}}^{(e)}(t)= \frac{\alpha_{j,\nu_{j}}^{(e)}}{\alpha_{j,\nu_{j}}^{(e)}-t}\label{eq:Mjnu_e}\\
%%% & \widetilde{M}_{j,\beta_{j}}^{(d,c)}(t)=\frac{\alpha_{j,\beta_{j}}^{(d)}(\alpha_{j,\beta_{j}}^{(c)}-t)}{\alpha_{j,\beta_{j}}^{(c)}(\alpha_{j,\beta_{j}}^{(d)}-t)},\,\,\,\forall j,\beta_{j}\label{eq:M_jbeta_dc}\\
%%%  & \alpha_{j,\beta_{j}}^{(d)}=w_{j,\beta_{j}}^{(d)}\alpha_{j}^{(d)},\,\,\,\forall j,\beta_{j}\label{eq:alpha_beta_d}\\
%%% & \alpha_{j,\beta_{j}}^{(c)}=w_{j,\beta_{j}}^{(c)}\alpha_{j}^{(c)},\,\,\,\forall j,\beta_{j}\label{eq:alpha_beta_c}\\
%%% & \alpha_{j,\nu_{j}}^{(e)}=w_{j,\nu_{j}}^{(e)}\alpha_{j}^{(e)},\,\,\,\forall j,\nu_{j}\label{eq:alpha_nu_e}\\
%%% & B_{j,\beta_{j}}^{(d)}(t)=\sum_{i=1}^{r}\frac{\lambda_{i}\pi_{i,j}q_{i,j,\beta_{j}}}{\Lambda_{j,\beta_{j}}^{(d)}}\left(\frac{\alpha_{j,\beta_{j}}^{(d)}}{\alpha_{j,\beta_{j}}^{(d)}-t}\right)^{L_{i}-L_{j,i}},\,\,\,\forall j,\beta_{j}\label{eq:Bjbeta_d}\\
%%% & B_{j,\beta_{j}}^{(c)}(t)=\sum_{i=1}^{r}\frac{\lambda_{i}\pi_{i,j}q_{i,j,\beta_{j}}}{\Lambda_{j,\beta_{j}}^{(c)}}\left(\frac{\alpha_{j,\beta_{j}}^{(c)}}{\alpha_{j,\beta_{j}}^{(c)}-t}\right)^{L_{i}-L_{j,i}},\,\,\,\forall j,\beta_{j}\label{eq:Bjbeta_c}\\
%%% & B_{j,\nu_{j}}^{(e)}(t)=\sum_{i=1}^{r}\frac{\lambda_{i}\pi_{i,j}p_{i,j,\nu_{j}}}{\Lambda_{j,\nu_{j}}^{(e)}}\left(\frac{\alpha_{j,\nu_{j}}^{(e)}}{\alpha_{j,\nu_{j}}^{(e)}-t}\right)^{L_{j,i}},\,\,\,\forall j,\nu_{j}\label{eq:Bjnu_e}\\
%%% & \rho_{j,\beta_{j}}^{(d)}=\sum_{i=1}^{r}\lambda_{i}\pi_{i,j}q_{i,j,\beta_{j}}\frac{L_{i}-L_{j,i}}{\alpha_{j,\beta_{j}}^{(d)}}<1,\,\,\,\forall j,\beta_{j}\label{eq:rho_beta_d}\\
%%% & \rho_{j,\beta_{j}}^{(c)}=\sum_{i=1}^{r}\lambda_{i}\pi_{i,j}q_{i,j,\beta_{j}}\frac{L_{i}-L_{j,i}}{\alpha_{j,\beta_{j}}^{(c)}}<1\,\forall j,\beta_{j}\label{eq:rho_beta_c}\\
%%% & \rho_{j,\nu_{j}}^{(e)}=\sum_{i=1}^{r}\lambda_{i}\pi_{i,j}p_{i,j,\nu_{j}}\frac{L_{j,i}}{\alpha_{j,\nu_{j}}^{(e)}}<1,\,\,\,\forall j,\nu_{j}\label{eq:rho_nu_e}
%% \end{align}
% 
% \vspace{-.1in}
% 
% \begin{align}
%&
%\sum_{i=1}^{r}\frac{\lambda_i}{\overline{\lambda}_i}\sum_{j=1}^{m}\pi_{i,j}\times\Biggl[\overline{c}+\widetilde{a}\,e^{-h_{i}\sigma}+\overline{a}\sum_{\nu_{j}=1}^{e_{j}}p_{i,j,\nu_{j}}\times\nonumber\nonumber \\
%& \sum_{\beta_{j}=1}^{d_{j}}q_{i,j,\beta_{j}}e^{h_{i}L_{i}\tau}\times\left(\delta^{(e)}+\delta^{(\overline{d})}+\delta^{(d,\overline{d})}\right)\label{eq:optfun}\\
% & \boldsymbol{\text{s.t.}}\nonumber\\
% &
%\eqref{alphad}-
%\eqref{Me_jnuj},\,
%\eqref{lambdac_betaj},\,
%\eqref{lambdae_nuj},\,
%\eqref{Be},
%%\eqref{rhoe},
%%\eqref{rhod},
%\eqref{Bd},
%%\eqref{rhoc},
%\eqref{Bc},
%\eqref{deltaAll}\label{formulas}\\ 
%&
%\widetilde{M}_{j,\beta_{j}}^{(d,\overline{d})}(h)=\frac{\alpha_{j,\beta_{j}}^{(d)}(\alpha_{j,\beta_{j}}^{(\overline{d})}-h)e^{\eta_{j,\beta_j}^{(d)}h}}{\alpha_{j,\beta_{j}}^{(\overline{d})}(\alpha_{j,\beta_{j}}^{(d)}-h)e^{\eta_{j,\beta_j}^{(\overline{d})}h}},\,\,\,\forall j,\beta_{j}\\
%& \rho_{j,\beta_{j}}^{(d)}=\sum_{i=1}^{r}\lambda_{i}\pi_{i,j}q_{i,j,\beta_{j}}e^{\lambda_i \omega_i}\frac{L_{i}-L_{j,i}}{\alpha_{j,\beta_{j}}^{(d)}}<1,\,\,\,\forall j,\beta_{j}\label{eq:rho_beta_d}\\
%& \rho_{j,\beta_{j}}^{(\overline{d})}=\sum_{i=1}^{r}\lambda_{i}\pi_{i,j}q_{i,j,\beta_{j}}e^{\lambda_i \omega_i}\frac{L_{i}-L_{j,i}}{\alpha_{j,\beta_{j}}^{(\overline{d})}}<1\,\forall j,\beta_{j}\label{eq:rho_beta_c}\\
%& \rho_{j,\nu_{j}}^{(e)}=\sum_{i=1}^{r}\lambda_{i}\pi_{i,j}p_{i,j,\nu_{j}}e^{\lambda_i \omega_i}\frac{L_{j,i}}{\alpha_{j,\nu_{j}}^{(e)}}<1,\,\,\,\forall j,\nu_{j}\label{eq:rho_nu_e}
%  \end{align}
%\begin{align}
%& \sum_{j=1}^{m}\pi_{i,j}=1,\,\,\,\forall i,\label{eq:sum_pi_ij}\\
%& \sum_{\nu_{j}=1}^{e_{j}}p_{i,,j,\nu_{j}}=1,\,\,\,\forall i,j\label{eq:sum_piij_nu}\\
%& \sum_{\beta_{j}=1}^{d_{j}}q_{i,,j,\beta_{j}}=1,\,\,\,\forall i,j\label{eq:sum_q_ij_beta}\\
% & \pi_{i,j},\,p_{i,,j,\nu_{j}},\,q_{i,,j,\beta_{j}}\geq0,\,\,\,\forall i,j,\beta_{j},\nu_{j}\label{eq:pi_q_p_gz}\\
%& w_{j,\beta_{j}}^{(\overline{d})},\,w_{j,\beta_{j}}^{(d)},\,w_{j,\nu_{j}}^{(e)}\geq0,\,\,\,\forall j,\beta_{j},\nu_{j}\label{eq:w_cde_gz}\\
%& \sum_{\beta_{j}=1}^{d_{j}}w_{j,\beta_{j}}^{(d)}\leq1,\,\,\,\forall j
%\label{eq:sum_w_d}\\
%& \sum_{\beta_{j}=1}^{d_{j}}w_{j,\beta_{j}}^{(\overline{d})}+\sum_{\nu_{j}=1}^{e_{j}}w_{j,\nu_{j}}^{(e)}\leq1,\,\,\,\forall j\label{eq:sum_w_de}\\
%& 
%\sum_{i}L_{j,i}\leq C_{j},\,L_{j,i}\geq0,\,\,\,\forall i,j\label{eq:capConst}\\
%& 
%\mathbb{P}(N_{j}>N_t)\leq \epsilon_j\label{P_N_j}\\
%& h_{i}<\alpha_{j,\beta_{j}}^{(d)},\,\,\,\forall i,j,\beta_{j}\label{eq:t_leq_alpha_beta_d}\\
%& h_{i}<\alpha_{j,\beta_{j}}^{(\overline{d})},\,\,\,\forall i,j,\beta_{j}\label{eq:t_leq_alpha_beta_c}\\
%& h_{i}<\alpha_{j,\nu_{j}}^{(e)},\,\,\,\forall i,j,\nu_{j}\label{eq:t_leq_alpha_nu_e}\\
% & 0<h_{i}-\Lambda_{j,\beta_{j}}^{(d)}(B_{j,\beta_{j}}^{(d)}(h_{i})-1),\,\,\,\forall i,j,\beta_{j}\label{eq:mgf_beta_d}\\
% & 0<h_{i}-\Lambda_{j,\beta_{j}}^{(\overline{d})}(B_{j,\beta_{j}}^{(\overline{d})}(h_{i})-1),\,\,\,\forall i,j,\beta_{j}\label{eq:mgf_beta_c}\\
% & 0<h_{i}-\Lambda_{j,\nu_{j}}^{(e)}(B_{j,\nu_{j}}^{(e)}(h_{i})-1),\,\,\,\forall i,j,\nu_{j}\label{eq:mgf_beta_e}\\
% &L_{j,i}\in {\mathbb Z}\label{eq:Lij}\\
%\boldsymbol{\text{var}} & \text{\,\,\,\,\,}\boldsymbol{\pi,}\,\boldsymbol{q},\,\boldsymbol{p},\,\boldsymbol{h},\,\boldsymbol{w}^{(c)},\,\boldsymbol{w}^{(d)},\,\boldsymbol{w}^{(e)},\,\boldsymbol{L}, \boldsymbol{\omega} \nonumber
%\end{align}
%
%{\bf Abubakr, there are ??, and some of the equations still may be cited from above, like the edge-cache utilization. Further, this needs index for the edge cache. }
%
%Here, the formulas mentioned in equation (\ref{formulas}) give the functions defined in the objective function. Constraints (\ref{eq:rho_beta_d})--(\ref{eq:rho_nu_e}) ensure the stability of the systems queue (do not blow up to infinity) while Constraints (\ref{eq:sum_pi_ij})--(\ref{eq:pi_q_p_gz}) guarantee that the two-stage probabilistic scheduling exists. Further, constraints (\ref{eq:w_cde_gz})--(\ref{eq:sum_w_de}) define the bandwidth split and ensure the feasibility of bandwidth allocation weights. Constraint (\ref{eq:capConst}) limits the cached segments to the storage server cache capacity. Constraint (\ref{P_N_j}) limits (with  $z^{th}$ percentile) the files in the edge-cache to not exceed $N_t$. Constraints (\ref{eq:t_leq_alpha_beta_d})--(\ref{eq:mgf_beta_e}) ensure that the moment generating functions exist. We note that some optimization variables can be combined to form a single optimization variable which results in having only five independent and separable variables as shown below. In the next subsection, we will describe the proposed algorithm for this optimization problem. 
%
%
%
%
%\subsection{Proposed Algorithm}
%\label{sec:algo}
%
%We first note that the two-stage probabilistic scheduling variables are independent and separable, thus we can combine them and define a single variable $\widetilde{\boldsymbol{\pi}}$ such that  
%$\widetilde{\boldsymbol{\pi}}=\left(\boldsymbol{\pi}\,,\boldsymbol{\,p}\,\,,\boldsymbol{q}\right)$. Similarly, since the bandwidth allocation weights are independent and separable, we concatenate them in a single optimization variable $\boldsymbol{w}$, where  
%$\boldsymbol{w}=\left(\boldsymbol{w}^{(e)}\,,\boldsymbol{\,w}^{(\overline{d})}\,\,,\boldsymbol{w}^{(d)}\right)$. Hence, the weighted SDTP optimization problem given in \eqref{eq:optfun}-\eqref{eq:Lij}  is optimized over five set of variables:  server and PSs scheduling probabilities $\widetilde{\boldsymbol{\pi}}$ (two-stage scheduling probabilities), auxiliary parameters $\boldsymbol{h}$, bandwidth allocation weights $\boldsymbol{w}$, and cache placement $\boldsymbol{L}$. 
%
%
% Clearly, the problem is non-convex in all the parameters jointly, which can be easily seen in the terms which are product of the different variables. Since the problem is non-convex, we propose an iterative algorithm to solve the problem. The proposed algorithm divides the problem into five sub-problems that optimize one variable while fixing the remaining four. These sub-problems are labeled as   (i) Server and PSs Access Optimization: optimizes  $\widetilde{\boldsymbol{\pi}}$, for given  $\boldsymbol{h}$, $\boldsymbol{w}$, $\boldsymbol{\omega}$, and $\boldsymbol{L}$,  
%(ii) Auxiliary Variables Optimization: optimizes  $\boldsymbol{h}$ for given $\widetilde{\boldsymbol{\pi}}$, $\boldsymbol{w}$, $\boldsymbol{\omega}$, and $\boldsymbol{L}$,  (iii) Bandwidth Allocation Optimization: optimizes  $\boldsymbol{w}$ for given $\widetilde{\boldsymbol{\pi}}$, $\boldsymbol{h}$, $\boldsymbol{\omega}$, and  $\boldsymbol{L}$. 
%(iv) Cache Placement Optimization: optimizes  $\boldsymbol{L}$ for given $\widetilde{\boldsymbol{\pi}}$, $\boldsymbol{h}$, $\boldsymbol{\omega}$, and $\boldsymbol{w}$, (v) Edge-cache Window Size Optimization: optimizes  $\boldsymbol{\omega}$ for given $\widetilde{\boldsymbol{\pi}}$, $\boldsymbol{h}$,  $\boldsymbol{L}$, and $\boldsymbol{w}$. The algorithm is summarized as follows. 
%
%%, where $\boldsymbol{\mathcal{S}}=\left(\mathcal{S}_{1},\mathcal{S}_{2},\ldots,\mathcal{S}_{r}\right)$,
%% (ii) access-scheduling probabilities  ($\boldsymbol{\pi}$- Optimization ), and finally (iii) auxiliary variables optimization ($\boldsymbol{t}$- Optimization). These sub-problems have an easier-to-handle structure and can be solved efficiently. Next, we develop an efficient algorithm solution for our optimization problem.
%%
%%
%%The joint mean-tail stall duration optimization problem given in (\ref{eq:joint_otp_prob}) is carried out over three set of variables: chunk placement $\mathcal{S}_{i}$, $\forall$ $i$, scheduling probabilities $\pi_{i,j}$, $\forall$ $i,j$, and auxiliary parameter $t_{i}$, $\forall$ $i$. In order to solve the non-convex problem, we develop an alternating minimization algorithm which is shown to converge to a stationary solution. The proposed algorithm can be written as follows.
%
%\begin{enumerate}[leftmargin=0cm,itemindent=.5cm,labelwidth=\itemindent,labelsep=0cm,align=left]
%\item \textbf{Initialization}: Initialize $\boldsymbol{h}$,\,$\widetilde{\boldsymbol{\pi}}$, $\boldsymbol{w}$, $\boldsymbol{\omega}$
%and $\boldsymbol{L}$ in the feasible set. 
%\item \textbf{While Objective Converges}
%\begin{enumerate}
%
%\item  Run Server Access Optimization using current values of $\boldsymbol{h}$, $\boldsymbol{w}$, $\boldsymbol{\omega}$, 
%and $\boldsymbol{L}$ to get new values of $\widetilde{\boldsymbol{\pi}}$
%
%
%\item  Run Auxiliary Variables Optimization using current values of $\widetilde{\boldsymbol{\pi}}$, $\boldsymbol{w}$, $\boldsymbol{\omega}$, 
%and $\boldsymbol{L}$ to get new values of $\boldsymbol{h}$
%
%
%
%\item  Run Bandwidth Allocation Optimization using current values
%of $\widetilde{\boldsymbol{\pi}}$, $\boldsymbol{h}$, $\boldsymbol{L}$, and $\boldsymbol{\omega}$, to get new values of $\boldsymbol{w}$. 
%
%
%\item  Run Cache Placement Optimization using current values
%of $\widetilde{\boldsymbol{\pi}}$, $\boldsymbol{h}$,   $\boldsymbol{w}$, and $\boldsymbol{\omega}$ to get new values of $\boldsymbol{L}$.
%
%
%\item  Run Edge-cache Window Size Optimization using current values
%of $\widetilde{\boldsymbol{\pi}}$, $\boldsymbol{h}$,   $\boldsymbol{w}$, and $\boldsymbol{L}$ to get new values of $\boldsymbol{\omega}$.
%
%\end{enumerate}
%\end{enumerate}
%
%%We next describe the five sub-problems along with the proposed solutions for the sub-problems.
%
%We next describe how our algorithm can be used in an online fashion to keep track of the systems dynamics at the edge-cache. 
%
%\input{online}
%
%
%%\textbf{Example:} add example to further illustrate. xxxx
\section{Optimization Problem Formulation and Proposed Algorithm }
\label{sec:SDTP}
\subsection{Problem Formulation}
We define 
%$\boldsymbol{\pi}=(\pi_{i,j}\forall i=1,\cdots,r\text{ and }j=1,\cdots,m)$,
%$\boldsymbol{p}=(p_{i,,j,\nu_{j}}\forall i=1,\cdots,r\,,j=1,\cdots,m\,,\,\nu_{j}=1,\ldots e_{j}),$
%$\boldsymbol{q}=(q_{i,,j,\beta_{j}}\forall i=1,\cdots,r\,,j=1,\cdots,m\,,\,\beta_{j}=1,\ldots d_{j}),$ $\boldsymbol{t}=\left(t_{1},t_{2},\ldots,t_{r}\right)$, 
%
%$\boldsymbol{w}_{j,\beta_{j}}^{(c)}=(w_{j,1}^{(c)},w_{j,2}^{(c)},\ldots,w_{j,d_{j}}^{(c)},\text{ and }j=1,\cdots,m)$,
%$\boldsymbol{w}_{j,\beta_{j}}^{(e)}=(w_{j,1}^{(e)},w_{j,2}^{(e)},\ldots,w_{j,d_{j}}^{(e)},\text{ and }j=1,\cdots,m)$,
%$\boldsymbol{w}_{j,\beta_{j}}^{(d)}=(w_{j,1}^{(d)},w_{j,2}^{(d)},\ldots,w_{j,d_{j}}^{(d)},\text{ and }j=1,\cdots,m)$,
%$\boldsymbol{L}_{j,i}=(L_{j,i},\,\forall i,\,\forall j)$
$\ensuremath{\ensuremath{\boldsymbol{\pi}=(\pi_{i,j,\ell}\forall i=1,\cdots,r\text{ and }j=1,\cdots,m,\ell=1,\cdots,R)},}\ensuremath{\boldsymbol{p}=(p_{i,,j,\nu_{j},\ell},(\nu_{j},\ell)\in\{(\nu_{j},\ell):\nu_{j}\in\{1,\ldots,e_{j}^{(\ell)}\},\ell\in\{1,\dots,R\}\},\forall i=1,\cdots,r\,,j=1,\cdots,m\,,\,\nu_{j}=1,\ldots e_{j}^{(\ell)},\ell=1,\cdots,R)},\ensuremath{\ensuremath{\boldsymbol{q}=(q_{i,,j,\beta_{j},\ell}\forall i=1,\cdots,r\,,j=1,\cdots,m\,,\,\beta_{j}=1,\ldots d_{j},\ell=1,\cdots,R)}},\ensuremath{\boldsymbol{h}=\left(h_{1},t_{2},\ldots,h_{r}\right)\,},\ensuremath{\ensuremath{\boldsymbol{w}^{(\overline{d})}=(w_{j,1,\ell}^{(\overline{d})},\ldots,w_{j,d_{j},\ell}^{(d)}\ensuremath{,}\text{ and }j=1,\cdots,m,\ell=1,\cdots,R)}\,,}\ensuremath{\boldsymbol{w}^{(e)}=(w_{j,1,\ell}^{(e)},w_{j,2,\ell}^{(e)},\ldots,w_{j,e_{j}^{(\ell)},\ell}^{(e)},\text{ and }j=1,\cdots,m,\ell=1,\ldots,R),\,}\ensuremath{\ensuremath{\boldsymbol{w}^{(d)}=(w_{j,1,\ell}^{(d)},\ldots,w_{j,d_{j},\ell}^{(d)},\text{ and }j=1,\cdots,m)}},\ensuremath{\boldsymbol{L}=(L_{j,i},\,\forall i=1,\,\text{ and }j=1,\cdots,m)}$
  and $\boldsymbol{\omega}=(\omega_{i,\ell}, \forall i,\ell)$.
Our goal is to minimize the SDTP  over the
choice of cache and datacenter access decisions, bandwidth allocation
weights, portion (number) of cached segments, time window over which we maintain the video files at edge-cache and auxiliary bound parameters.

To incorporate for weighted fairness and differentiated services,
we assign a positive weight $\kappa_{i,\ell}$ for each file $i$. Without
loss of generality, each file $i$ is weighted by the arrival rate
$\lambda_{i,\ell}$ in the objective (so larger arrival rates are weighted
higher). However, any other weights can be incorporated to accommodate
for weighted fairness or differentiated services. Let $\overline{\lambda}=\sum_{i,\ell}\lambda_{i,\ell}$
be the total arrival rate. Hence, $\kappa_{i,\ell}=\lambda_{i,\ell}/\overline{\lambda}$
is the ratio of file $i$ requests. Hence, the objective is the minimization
of stall duration tail probability, averaged over all the file requests,
and is given as $\sum_{i,\ell}\frac{\lambda_{i,\ell}}{\overline{\lambda}}\,\text{\text{Pr}}\left(\Gamma^{(i)}\geq\sigma\right)$.
By using the expression for SDTP in Section \ref{sec:StallTailProb},
the optimization problem can be formulated as follows.
%\begin{align}
%%\text{\textbf{min}\,\,\,\,\,}\sum_{i=1}^{r}\frac{\lambda_{i}}{\overline{\lambda}} & \sum_{j=1}^{m}\pi_{i,j}\left[e^{-t_{i}\sigma}+\sum_{\nu_{j}=1}^{e_{j}}p_{i,j,\nu_{j}}e^{(\widetilde{\sigma}-\overline{\sigma})t_{i}}\frac{M_{j,\nu_{j}}^{(e)}(t_i)(1-\rho_{j,\nu_{j}}^{(e)})t_iB_{j,\nu_{j}}^{(e)}(t_i)}{t_i-\Lambda_{j,\nu_{j}}^{(e)}(B_{j,\nu_{j}}^{(e)}(t_i)-1)}\frac{\left((M_{j,\nu_{j}}^{(e)}(t_i))^{L_{j,i}}-1\right)}{M_{j,\nu_{j}}^{(e)}(t_i)-1}\right. \nonumber \\
%%& +\sum_{\beta_{j}=1}^{d_{j}}q_{i,j,\beta_{j}}e^{(\widetilde{\sigma}-\overline{\sigma})t_{i}}\frac{(1-\rho_{j,\beta_{j}}^{(c)})t_iB_{j,\beta_{j}}^{(c)}(t_i)}{t_i-\Lambda_{j,\beta_{j}}^{(c)}(B_{j,\beta_{j}}^{(c)}(t_i)-1)}\left(\frac{\alpha_{j,\beta_{j}}^{(c)}}{\alpha_{j,\beta_{j}}^{(c)}-t_i}\right)^{L_{i}-L_{j,i}} (L_i - L_{j,i})\nonumber \\
%%& +  \sum_{\beta_{j}=1}^{d_{j}}q_{i,j,\beta_{j}}e^{(\widetilde{\sigma}-\overline{\sigma})t_{i}}\frac{(1-\rho_{j,\beta_{j}}^{(d)})t_iB_{j,\beta_{j}}^{(d)}(t_i) \left(\widetilde{M}_{j,\beta_{j}}^{(d,c)}(t_i)\right)^{L_{j,i}+1}}{t_i-\Lambda_{j,\beta_{j}}^{(d)}(B_{j,\beta_{j}}^{(d)}(t_i)-1)}\left(\frac{\alpha_{j,\beta_{j}}^{(d)}-t_i}{\alpha_{j,\beta_{j}}^{(d)}}\right)^{L_{j,i}+1}\left(\frac{\alpha_{j,\beta_{j}}^{(c)}}{\alpha_{j,\beta_{j}}^{(c)}-t_i}\right)^{L_{i}+1} \nonumber\\
%%& \left.  \left(\frac{\left(\widetilde{M}_{j,\beta_{j}}^{(d,c)}(t_i)\right)^{L_i-L_{j,i}}-(L_i-L_{j,i})}{\widetilde{M}_{j,\beta_{j}}^{(d,c)}(t_i)-1}+ \frac{\widetilde{M}_{j,\beta_{j}}^{(d,c)}(t_i)\left(\left(\widetilde{M}_{j,\beta_{j}}^{(d,c)}(t_i)\right)^{L_i-L_{j,i}-1}-1\right)}{\left(\widetilde{M}_{j,\beta_{j}}^{(d,c)}(t_i)-1\right)^2}\right)\right]label\label{eq:optfun}\\
%%\boldsymbol{\text{s.t.}}\nonumber \\
%% & \Lambda_{j,\beta_{j}}^{(d)}=\sum_{i=1}^{r}\lambda_{i}\pi_{i,j}q_{i,j,\beta_{j}},\,\,\,\forall j,\beta_{j}\label{eq:Lamda_d}\\
%% & \Lambda_{j,\beta_{j}}^{(c)}=\sum_{i=1}^{r}\lambda_{i}\pi_{i,j}q_{i,j,\beta_{j}},\,\,\,\forall j,\beta_{j}\label{eq:Lamda_c}\\
%% & \Lambda_{j,\nu_{j}}^{(e)}=\sum_{i=1}^{r}\lambda_{i}\pi_{i,j}p_{i,j,\nu_{j}},\,\,\,\forall j,\nu_{j}\label{eq:Lamda_e}\\
%% & M_{j,\nu_{j}}^{(e)}(t)= \frac{\alpha_{j,\nu_{j}}^{(e)}}{\alpha_{j,\nu_{j}}^{(e)}-t}\label{eq:Mjnu_e}\\
%% & \widetilde{M}_{j,\beta_{j}}^{(d,c)}(t)=\frac{\alpha_{j,\beta_{j}}^{(d)}(\alpha_{j,\beta_{j}}^{(c)}-t)}{\alpha_{j,\beta_{j}}^{(c)}(\alpha_{j,\beta_{j}}^{(d)}-t)},\,\,\,\forall j,\beta_{j}\label{eq:M_jbeta_dc}\\
%%  & \alpha_{j,\beta_{j}}^{(d)}=w_{j,\beta_{j}}^{(d)}\alpha_{j}^{(d)},\,\,\,\forall j,\beta_{j}\label{eq:alpha_beta_d}\\
%% & \alpha_{j,\beta_{j}}^{(c)}=w_{j,\beta_{j}}^{(c)}\alpha_{j}^{(c)},\,\,\,\forall j,\beta_{j}\label{eq:alpha_beta_c}\\
%% & \alpha_{j,\nu_{j}}^{(e)}=w_{j,\nu_{j}}^{(e)}\alpha_{j}^{(e)},\,\,\,\forall j,\nu_{j}\label{eq:alpha_nu_e}\\
%% & B_{j,\beta_{j}}^{(d)}(t)=\sum_{i=1}^{r}\frac{\lambda_{i}\pi_{i,j}q_{i,j,\beta_{j}}}{\Lambda_{j,\beta_{j}}^{(d)}}\left(\frac{\alpha_{j,\beta_{j}}^{(d)}}{\alpha_{j,\beta_{j}}^{(d)}-t}\right)^{L_{i}-L_{j,i}},\,\,\,\forall j,\beta_{j}\label{eq:Bjbeta_d}\\
%% & B_{j,\beta_{j}}^{(c)}(t)=\sum_{i=1}^{r}\frac{\lambda_{i}\pi_{i,j}q_{i,j,\beta_{j}}}{\Lambda_{j,\beta_{j}}^{(c)}}\left(\frac{\alpha_{j,\beta_{j}}^{(c)}}{\alpha_{j,\beta_{j}}^{(c)}-t}\right)^{L_{i}-L_{j,i}},\,\,\,\forall j,\beta_{j}\label{eq:Bjbeta_c}\\
%% & B_{j,\nu_{j}}^{(e)}(t)=\sum_{i=1}^{r}\frac{\lambda_{i}\pi_{i,j}p_{i,j,\nu_{j}}}{\Lambda_{j,\nu_{j}}^{(e)}}\left(\frac{\alpha_{j,\nu_{j}}^{(e)}}{\alpha_{j,\nu_{j}}^{(e)}-t}\right)^{L_{j,i}},\,\,\,\forall j,\nu_{j}\label{eq:Bjnu_e}\\
%% & \rho_{j,\beta_{j}}^{(d)}=\sum_{i=1}^{r}\lambda_{i}\pi_{i,j}q_{i,j,\beta_{j}}\frac{L_{i}-L_{j,i}}{\alpha_{j,\beta_{j}}^{(d)}}<1,\,\,\,\forall j,\beta_{j}\label{eq:rho_beta_d}\\
%% & \rho_{j,\beta_{j}}^{(c)}=\sum_{i=1}^{r}\lambda_{i}\pi_{i,j}q_{i,j,\beta_{j}}\frac{L_{i}-L_{j,i}}{\alpha_{j,\beta_{j}}^{(c)}}<1\,\forall j,\beta_{j}\label{eq:rho_beta_c}\\
%% & \rho_{j,\nu_{j}}^{(e)}=\sum_{i=1}^{r}\lambda_{i}\pi_{i,j}p_{i,j,\nu_{j}}\frac{L_{j,i}}{\alpha_{j,\nu_{j}}^{(e)}}<1,\,\,\,\forall j,\nu_{j}\label{eq:rho_nu_e}
% \end{align}
\vspace{-.1in}
\begin{align}
&
\sum_{\ell=1}^{R}\sum_{i=1}^{r}\frac{\lambda_{i,\ell}}{\overline{\lambda}_{i,\ell}}\sum_{j=1}^{m}\pi_{i,j,\ell}\times\Biggl[\overline{c}_{\ell}+\widetilde{a}_{\ell}\,e^{-h_{i}\sigma}+\overline{a}_{\ell}\sum_{\nu_{j}=1}^{e_{j}}p_{i,j,\nu_{j},\ell}\times\nonumber\nonumber \\
& \sum_{\beta_{j}=1}^{d_{j}}q_{i,j,\beta_{j},\ell}e^{h_{i}L_{i}\tau}\times\left(\delta^{(e)}+\delta^{(\overline{d})}+\delta^{(d,\overline{d})}\right)\label{eq:optfun}\\
& \boldsymbol{\text{s.t.}}\nonumber\\
&
\eqref{sumWs}-\eqref{lambdae_nuj},\eqref{edgeCacheConst}, \eqref{deltae}-\eqref{eq:abar}
%\eqref{alphad}-
%\eqref{Me_jnuj},\,
%\eqref{lambdac_betaj},\,
%\eqref{lambdae_nuj},\,
%\eqref{edgeCacheConst},\,
%%\eqref{Be},
%%\eqref{rhod},
%%\eqref{Bd},
%%\eqref{rhoc},
%\eqref{eq:delta_e}-\eqref{eq:mgf_dpar}
%%\eqref{Bc},
%%\eqref{deltaAll}
\label{formulas}
\\ 
%&
%\widetilde{M}_{j,\beta_{j},\ell}^{(d,\overline{d})}(h)=\frac{\alpha_{j,\beta_{j},\ell}^{(d)}(\alpha_{j,\beta_{j},\ell}^{(\overline{d})}-h)e^{\eta_{j,\beta_j,\ell}^{(d)}h}}{\alpha_{j,\beta_{j},\ell}^{(\overline{d})}(\alpha_{j,\beta_{j},\ell}^{(d)}-h)e^{\eta_{j,\beta_j,\ell}^{(\overline{d})}h}},\,\,\,\forall j,\beta_{j}\\
& \rho_{j,\beta_{j},\ell}^{(d)}=\sum_{i=1}^{r}\lambda_{i,\ell}\pi_{i,j}q_{i,j,\beta_{j},\ell}e^{\lambda_{i,\ell} \omega_{i,\ell}}\frac{L_{i}-L_{j,i}}{\alpha_{j,\beta_{j},\ell}^{(d)}}<1,\,\,\,\forall j,\beta_{j}\label{eq:rho_beta_d}\\
& \rho_{j,\beta_{j},\ell}^{(\overline{d})}=\sum_{i=1}^{r}\lambda_{i,\ell}\pi_{i,j,\ell}q_{i,j,\beta_{j},\ell}e^{\lambda_{i,\ell} \omega_{i,\ell}}\frac{L_{i}-L_{j,i}}{\alpha_{j,\beta_{j},\ell}^{(\overline{d})}}<1\,\forall j,\beta_{j},\ell\label{eq:rho_beta_c}\\
& \rho_{j,\nu_{j},\ell}^{(e)}=\sum_{i=1}^{r}\lambda_{i,\ell}\pi_{i,j,\ell}p_{i,j,\nu_{j},\ell}e^{\lambda_{i,\ell} \omega_{i,\ell}}\frac{L_{j,i}}{\alpha_{j,\nu_{j},\ell}^{(e)}}<1,\,\,\,\forall j,\nu_{j},\ell\label{eq:rho_nu_e}
\end{align}

\begin{align}
%& \sum_{j=1}^{m}\pi_{i,j,\ell}=1,\,\,\,\forall i,\ell \label{eq:sum_pi_ij}\\
%& \sum_{\nu_{j}=1}^{e_{j}}p_{i,,j,\nu_{j},\ell}=1,\,\,\,\forall i,j,\ell \label{eq:sum_piij_nu}\\
%& \sum_{\beta_{j}=1}^{d_{j}}q_{i,j,\beta_{j},\ell}=1,\,\,\,\forall i,j,\ell\label{eq:sum_q_ij_beta}\\
%& \pi_{i,j,\ell},\,p_{i,,j,\nu_{j},\ell},\,q_{i,,j,\beta_{j},\ell}\geq0,\,\,\,\forall i,j,\beta_{j},\nu_{j},\ell\label{eq:pi_q_p_gz}\\
%& w_{j,\beta_{j},\ell}^{(\overline{d})},\,w_{j,\beta_{j}}^{(d)},\,w_{j,\nu_{j},\ell}^{(e)}\geq0,\,\,\,\forall j,\beta_{j},\nu_{j},\ell\label{eq:w_cde_gz}\\
%& \sum_{\beta_{j}=1}^{d_{j}}w_{j,\beta_{j}}^{(d)}\leq1,\,\,\,\forall j
%\label{eq:sum_w_d}\\
%& \sum_{\beta_{j}=1}^{d_{j}}w_{j,\beta_{j},\ell}^{(\overline{d})}+\sum_{\nu_{j}=1}^{e_{j}}w_{j,\nu_{j},\ell}^{(e)}\leq1,\,\,\,\forall j,\ell\label{eq:sum_w_de}\\
& 
\sum_{i}L_{j,i}\leq C_{j},\,L_{j,i}\geq0,\,\,\,\forall i,j\label{eq:capConst}\\
%& 
%\mathbb{P}(N_{\ell}>N_t)\leq \epsilon_{\ell}\label{P_N_j}\\
& h_{i}<\alpha_{j,\beta_{j}}^{(d)},
%
%\,\,\,\forall i,j,\beta_{j}
%\label{eq:t_leq_alpha_beta_d}
%&
h_{i}<\alpha_{j,\beta_{j},\ell}^{(\overline{d})},
%\,\,\,\forall i,j,\beta_{j},\ell\
%label{eq:t_leq_alpha_beta_c}
%&
h_{i}<\alpha_{j,\nu_{j},\ell}^{(e)},\,\,\,\forall i,j,\nu_{j},\ell \label{eq:t_leq_alpha_nu_e}\\
& 
0<h_{i}-\Lambda_{j,\beta_{j}}^{(d)}(B_{j,\beta_{j},\ell}^{(d)}(h_{i})-1),\,\,\,\forall i,j,\beta_{j},\ell\label{eq:mgf_beta_d}\\
& 0<h_{i}-\Lambda_{j,\beta_{j},\ell}^{(\overline{d})}(B_{j,\beta_{j},\ell}^{(\overline{d})}(h_{i})-1),\,\,\,\forall i,j,\beta_{j}\label{h_const}\\
& 0<h_{i}-\Lambda_{j,\nu_{j},\ell}^{(e)}(B_{j,\nu_{j},\ell}^{(e)}(h_{i})-1),\,\,\,\forall i,j,\nu_{j},\ell\label{eq:mgf_beta_e}\\
&L_{j,i}\in {\mathbb Z}\label{eq:Lij}\\
\boldsymbol{\text{var}} & \text{\,\,\,\,\,}\boldsymbol{\pi,}\,\boldsymbol{q},\,\boldsymbol{p},\,\boldsymbol{h},\,\boldsymbol{w}^{(c)},\,\boldsymbol{w}^{(d)},\,\boldsymbol{w}^{(e)},\,\boldsymbol{L}, \boldsymbol{\omega} \nonumber
\end{align}

%{\bf Abubakr, there are ??, and some of the equations still may be cited from above, like the edge-cache utilization. Further, this needs index for the edge cache. }

Here, in (\ref{formulas}), equations $(1)-(3)$ give the feasibility constraints on the bandwidth allocation, while equations $(4)-(6)$ define the MGFs of the service time distributions, equations $(7)-(10)$ give the feasibility of the two-stage probabilistic scheduling and $(11)-(12)$ define the arrival rates at the different queues. Constraints 
(\ref{eq:rho_beta_d})--(\ref{eq:rho_nu_e}) ensure the stability of the systems queue (do not blow up to infinity).
% while Constraints (\ref{eq:sum_pi_ij})--(\ref{eq:pi_q_p_gz}) guarantee that the two-stage probabilistic scheduling exists. 
% 
% Further, constraints (\ref{eq:w_cde_gz})--(\ref{eq:sum_w_de}) define the bandwidth split and ensure the feasibility of bandwidth allocation weights.
%Constraint (\ref{eq:capConst}) limits the cached segments to the storage server cache capacity. Constraint (\ref{P_N_j}) limits (with  $z^{th}$ percentile) the files in the edge-cache to not exceed $N_t$. The exact expression for this constraint is given in \eqref{edgeCacheConst}. 
Constraints (\ref{eq:t_leq_alpha_nu_e})--(\ref{eq:mgf_beta_e}) ensure that the moment generating functions exist. We note that some optimization variables can be combined to form a single optimization variable which results in having only five independent and separable variables as shown below. In the next subsection, we will describe the proposed algorithm for this optimization problem. 
\subsection{Proposed Algorithm}
\label{sec:algo}

We first note that the two-stage probabilistic scheduling variables are independent and separable, thus we can combine them and define a single variable $\widetilde{\boldsymbol{\pi}}$ such that  
$\widetilde{\boldsymbol{\pi}}=\left(\boldsymbol{\pi}\,,\boldsymbol{\,p}\,\,,\boldsymbol{q}\right)$. Similarly, since the bandwidth allocation weights are independent and separable, we concatenate them in a single optimization variable $\boldsymbol{w}$, where  
$\boldsymbol{w}=\left(\boldsymbol{w}^{(e)}\,,\boldsymbol{\,w}^{(\overline{d})}\,\,,\boldsymbol{w}^{(d)}\right)$. Hence, the weighted SDTP optimization problem given in \eqref{eq:optfun}-\eqref{eq:Lij}  is optimized over five set of variables:  server and PSs scheduling probabilities $\widetilde{\boldsymbol{\pi}}$ (two-stage scheduling probabilities), auxiliary parameters $\boldsymbol{h}$, bandwidth allocation weights $\boldsymbol{w}$, cache placement $\boldsymbol{L}$, and edge cache window size optimization $\boldsymbol{\omega}$. 


Clearly, the problem is non-convex in all the parameters jointly, which can be easily seen in the terms which are product of the different variables. Since the problem is non-convex, we propose an iterative algorithm to solve the problem. The proposed algorithm divides the problem into five sub-problems that optimize one variable while fixing the remaining four. These sub-problems are labeled as   (i) Server and PSs Access Optimization: optimizes  $\widetilde{\boldsymbol{\pi}}$, for given  $\boldsymbol{h}$, $\boldsymbol{w}$, $\boldsymbol{\omega}$, and $\boldsymbol{L}$,  
(ii) Auxiliary Variables Optimization: optimizes  $\boldsymbol{h}$ for given $\widetilde{\boldsymbol{\pi}}$, $\boldsymbol{w}$, $\boldsymbol{\omega}$, and $\boldsymbol{L}$,  (iii) Bandwidth Allocation Optimization: optimizes  $\boldsymbol{w}$ for given $\widetilde{\boldsymbol{\pi}}$, $\boldsymbol{h}$, $\boldsymbol{\omega}$, and  $\boldsymbol{L}$. 
(iv) Cache Placement Optimization: optimizes  $\boldsymbol{L}$ for given $\widetilde{\boldsymbol{\pi}}$, $\boldsymbol{h}$, $\boldsymbol{\omega}$, and $\boldsymbol{w}$, (v) Edge-cache Window Size Optimization: optimizes  $\boldsymbol{\omega}$ for given $\widetilde{\boldsymbol{\pi}}$, $\boldsymbol{h}$,  $\boldsymbol{L}$, and $\boldsymbol{w}$. The algorithm is summarized as follows. 

%, where $\boldsymbol{\mathcal{S}}=\left(\mathcal{S}_{1},\mathcal{S}_{2},\ldots,\mathcal{S}_{r}\right)$,
% (ii) access-scheduling probabilities  ($\boldsymbol{\pi}$- Optimization ), and finally (iii) auxiliary variables optimization ($\boldsymbol{t}$- Optimization). These sub-problems have an easier-to-handle structure and can be solved efficiently. Next, we develop an efficient algorithm solution for our optimization problem.
%
%
%The joint mean-tail stall duration optimization problem given in (\ref{eq:joint_otp_prob}) is carried out over three set of variables: chunk placement $\mathcal{S}_{i}$, $\forall$ $i$, scheduling probabilities $\pi_{i,j}$, $\forall$ $i,j$, and auxiliary parameter $t_{i}$, $\forall$ $i$. In order to solve the non-convex problem, we develop an alternating minimization algorithm which is shown to converge to a stationary solution. The proposed algorithm can be written as follows.

\begin{enumerate}[leftmargin=0cm,itemindent=.5cm,labelwidth=\itemindent,labelsep=0cm,align=left]
	\item \textbf{Initialization}: Initialize $\boldsymbol{h}$,\,$\widetilde{\boldsymbol{\pi}}$, $\boldsymbol{w}$, $\boldsymbol{\omega}$
	and $\boldsymbol{L}$ in the feasible set. 
	\item \textbf{While Objective Converges}
	\begin{enumerate}
		
		\item  Run Server Access Optimization using current values of $\boldsymbol{h}$, $\boldsymbol{w}$, $\boldsymbol{\omega}$, 
		and $\boldsymbol{L}$ to get new values of $\widetilde{\boldsymbol{\pi}}$
		
		
		\item  Run Auxiliary Variables Optimization using current values of $\widetilde{\boldsymbol{\pi}}$, $\boldsymbol{w}$, $\boldsymbol{\omega}$, 
		and $\boldsymbol{L}$ to get new values of $\boldsymbol{h}$
		
		
		
		\item  Run Bandwidth Allocation Optimization using current values
		of $\widetilde{\boldsymbol{\pi}}$, $\boldsymbol{h}$, $\boldsymbol{L}$, and $\boldsymbol{\omega}$, to get new values of $\boldsymbol{w}$. 
		
		
		\item  Run Cache Placement Optimization using current values
		of $\widetilde{\boldsymbol{\pi}}$, $\boldsymbol{h}$,   $\boldsymbol{w}$, and $\boldsymbol{\omega}$ to get new values of $\boldsymbol{L}$.
		
		
		\item  Run Edge-cache Window Size Optimization using current values
		of $\widetilde{\boldsymbol{\pi}}$, $\boldsymbol{h}$,   $\boldsymbol{w}$, and $\boldsymbol{L}$ to get new values of $\boldsymbol{\omega}$.
		
	\end{enumerate}
\end{enumerate}


The proposed algorithm performs an alternating optimization over the different aforementioned dimensions, such that each sub-problem is shown to have convex constraints and thus can be efficiently solved using the iNner cOnVex Approximation (NOVA)  algorithm proposed in \cite{scutNOVA}. The subproblems are explained in detailed in Appendix \ref{opt_mention}. 

%\subsubsection*{Convergence of the Proposed Algorithm}

We first initialize 
$\widetilde{\boldsymbol{\pi}}$, $\boldsymbol{w}$, $\boldsymbol{h}$, $\boldsymbol{\omega}$, and $\boldsymbol{L}$ $\forall i, j, \nu_j, \beta_j$ such that the choice is feasible for the problem. Then, we do alternating minimization over the five sub-problems defined above. Since each sub-problem can only decrease the objective (properties of convergence of subproblems to a stationary point is given in Appendix \ref{opt_mention}) and the overall problem is bounded from below, we have the following result.

\begin{theorem} 
	The proposed algorithm  converges to a  stationary solution.
\end{theorem}

%We next describe the five sub-problems along with the proposed solutions for the sub-problems.
Appendix \ref{sec:adapt}  describes how our algorithm can be used in an online fashion to keep track of the systems dynamics at the edge-cache. 

%Next, we present our evaluation results for our proposed scheme considering both offline and online versions of our proposed algorithm. 


%\textbf{Example:} add example to further illustrate. xxxx

==> results.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure}[t]
	\centering
	\includegraphics[trim=0in 0in 0in 0.0in, clip, width=.48\textwidth]{figs2/stallconvrg_final}
			\vspace{-.16in}
		\captionof{figure}{Convergence of mean stall duration.}
		\label{fig:ConvgMeanStall}
		\vspace{-.2in}
\end{figure}




\begin{figure*}
	\centering
	\begin{minipage}{.32\textwidth}
		\centering
		\includegraphics[trim=0in 0in 4.1in 0in, clip, width=\textwidth]{figs2/stall_vs_ArrRate_final}
%		\vspace{-.3in}
		\captionof{figure}{Mean stall duration for different video arrival rates.}
		\label{fig:meanStallVsArrRate}
	\end{minipage}%
	\hspace{2mm}
	\begin{minipage}{.32\textwidth}
		\centering
		\includegraphics[trim=0.1in 0in 4in 0in, clip, width=\textwidth]{figs2/qlty_vs_arrRate_final}
%		\vspace{-.3in}
		\captionof{figure}{Average quality for different video arrival rates.}
		\label{fig:meanQltyVsArrRate}
	\end{minipage}
	\hspace{2mm}
	\begin{minipage}{.32\textwidth}
		\centering
		\includegraphics[trim=0in 0in 4in 0in, clip,width=\textwidth]{figs2/stall_vs_VidSize_final}
%		\vspace{-.3in}
		\captionof{figure}{Mean stall duration for different video lengths.}
		\label{fig:meanStallVsVidSize} 
	\end{minipage}
%	\vspace{-.2in}
	\centering
	\begin{minipage}{.32\textwidth}
		\centering
		\includegraphics[trim=0.1in 0in 4.8in 0in, clip, width=\textwidth]{figs2/qlty_vs_vidLen_final_v2}
%		\vspace{-.3in}
		\captionof{figure}{Average  quality for different video lengths.}
		\label{fig:meanQltyVsVidSize}
	\end{minipage}%
	\hspace{2mm}
	\begin{minipage}{.32\textwidth}
		\centering
		\includegraphics[trim=0.0in 0in 3.8in 0in, clip, width=\textwidth]{figs2/qulty_stall_vs_VM_dj}
%		\vspace{-.3in}
		\captionof{figure}{Average video quality and mean stall duration for different number of parallel streams $d_j$.}
		\label{fig:qlty_stall_Vs_d_j}
	\end{minipage}
	\hspace{2mm}
	\begin{minipage}{.32\textwidth}
		\centering
		\includegraphics[trim=0.1in 0.1in 4.4in 0.1in, clip,width=\textwidth]{figs2/tradeOff_final_v2}
%		\vspace{-.3in}
		\captionof{figure}{Tradeoff between mean stall duration and  average streamed video quality obtained by varying $\theta$.}
		\vspace{-.15in}
		\label{fig:tradeoff} 
	\end{minipage}
%	\vspace{-.2in}


\end{figure*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%













%\begin{figure}[t].
%		\centering
%	\includegraphics[trim=0.1in 0in 0.0in 0in, clip, scale =0.35]{figs/stall_vs_ArrRate_all}
%			\vspace{-.2in}
%		\captionof{figure}{Mean stall duration for different video arrival rates. }
%		\label{fig:meanStallVsArrRate}
%		\vspace{-.18in}
%\end{figure}
%
%\begin{figure}[t]
%		\centering		\includegraphics[trim=0.1in 0in 0.0in 0.0in, clip,scale =0.35]{figs/qlty_vs_ArrRate_all}
%				\vspace{-.2in}
%		\captionof{figure}{Average quality for different video arrival rates.}
%		\label{fig:meanQltyVsArrRate}
%		\vspace{-.18in}
%\end{figure}


%\subsection{Mean Stall Duration optimization}
%In this subsection, we focus only on minimizing the mean stall duration of all files by setting $\theta=1$, {\em i.e.}, stall duration tail probability is not considered.% in this part of the simulation.

\subsubsection*{Convergence of the Proposed Algorithm}
Figure \ref{fig:ConvgMeanStall} shows the convergence  of our proposed algorithm, where we see the convergence of mean stall duration in about $2000$ iterations. 

% which alternatively optimizes the mean stall duration of all files over scheduling probabilities $\boldsymbol{\pi}$, auxiliary variables $\boldsymbol{t}$, quality probabilities $\boldsymbol{b}$, and bandwidth allocation weights $\boldsymbol{w}$. We notice that for $r=1000$ video files of size 600 sec with $m=12$ storage nodes and six quality levels shown in \ref{tab:DataRates}, the mean stall duration converges to the optimal value within less than $300$ iterations.  


\subsubsection*{Effect of Arrival Rate} We assume the arrival rate of all the files the same, and vary the arrival rates as depicted in Figures \ref{fig:meanStallVsArrRate} and \ref{fig:meanQltyVsArrRate}. These figures show the effect of different video arrival rates on the mean stall duration and  averaged quality, respectively. We note that PLQ-BTA achieves lowest stalls and lowest quality, since it fetches all videos at the lowest qualities. Similarly, PHQ-BTA has highest stalls, and highest video quality since it fetches all videos in the highest possible rate. The proposed algorithm has mean stall duration less than all the algorithms other than PLQ-BTA, and is very close to PLQ-BTA.  Further, the proposed algorithm has the highest video quality among all algorithms except PHQ-BTA and PEQ-BTA. Thus, the proposed algorithm helps optimize both the QoEs simultaneously achieving close to the best possible stall durations and achieving better average video quality than the baselines. With the choice of low $\theta$, the stall duration can be made very close to the stall duration achieved with the lowest quality while the proposed algorithm will still opportunistically increase quality of certain videos to obtain better average quality. 



%We compare our proposed algorithm with the six baseline  policies and see that the proposed algorithm outperforms all baseline strategies for the QoE metrics of mean stall duration and  average quality. Thus, sever access, VMs selection and bandwidth weights allocation of files are important for the reduction of mean stall duration. While the mean stall duration increases with arrival, our approach still maintain low mean stall duration compared to the baselines. Moreover, we observe that the algorithms that optimize the quality tend to increase the quality of the streamed video only if the stall durations are zero (or close to zero) and adopt the lowest quality if the stall durations are not zero.
%Figure \ref{fig:meanQltyVsArrRate}
%shows that PLQ-BTA (PHQ-BTA) streaming policy realizes the lowest (highest) mean stall duration as it is aggressively minimize (maximize) the stall (quality) at the cost of other optimized parameters.


%Intuitively, having optimized placement leads to less stall duration (for all policies) since video chunks are balanced across the different storage nodes. Hence, the possibility of congested bottleneck nodes reduces accordingly. While mean stall duration increases as arrival rate increases, our approach, unlike PEAP and BNW, does not explode  as others do (especially for optimized one). 

\subsubsection*{Effect of Video Length}
The effect of having different video lengths on the mean stall duration and  average quality is also captured in Figures \ref{fig:meanStallVsVidSize} and \ref{fig:meanQltyVsVidSize}, respectively, where we assume that all the videos are of the same length. Apparently, the mean stall duration increases with the video length while the average quality decreases with the video length. The qualitative comparison of the different algorithms is the same as described in the case of varying arrival rates. Thus, at $\theta = 10^{-7}$, the proposed algorithm achieves the mean stall duration close to that of  PLQ-BTA while achieving significantly better quality. For algorithms other than PLQ-BTA, PEQ-BTA, and PHQ-BTA, the proposed algorithms outperforms all other baselines in both the metrics. %We also note that a fixed $\theta$ is used, and thus the average quality term gets more preference as the video lengths increase. Thus, for higher video lengths, 



%larger video sizes may incur more stalls as compared to the small ones since the chance of getting delayed chunks is increased. However, our proposed approach gives the lowest mean stall duration compared to the considered baselines. Since we magnify stall minimization over quality enhancement, the controlled-quality based algorithms stream the video with base-layer (the lowest possible) quality when the stalls are not equal to zero and stream with higher quality only if the stalls are zero. The greedy-based approaches (PLQ-BTA and PHQ-BTA) look into one metric to signify without taking the another one into account which results in performing the worst among all other algorithms with respect to the non-optimized parameter. For example, PHQ-BTA achieves the highest quality but, on the hand, realizes the highest mean stall duration. Finally, we note that the proposed optimization strategy effectively reduces the mean stall duration (while maintaining smooth streamed video) and outperforms the considered baseline strategies. Thus, joint optimization over all optimized parameters helps reduce the mean stall duration significantly and optimize the  average quality.


%\begin{figure}[t]
%\includegraphics[scale=0.55]{figures2/Fig_7_mean_stall_NoOfFiles_source.eps}
%\caption{Mean stall duration for different number of video files with different video sizes. \label{fig:meanStallNumFiles} }
%\end{figure}


%\subsubsection*{Effect of the Number of Video Files}
%
%Figure \ref{fig:meanStallNumFiles} demonstrates the impact of varying the number of video files from $200$ files to $1000$ files  on the mean stall duration, where the video lengths are generated according to Pareto distribution with the same parameter defined earlier (scale of 300, and shape of 2).  We note that the proposed optimization strategy effectively reduces the mean stall duration and outperforms the considered baseline strategies. Thus, joint optimization over all three variables $\boldsymbol{t}$,  $\boldsymbol{\pi}$,  $\boldsymbol{w}$, and  $\boldsymbol{b}$ helps reduce the mean stall duration significantly.


%\subsection{Average Quality  Optimization}
%
%In this subsection, we consider optimizing (magnifying) the quality of the streamed video by maximizing the quality probabilities, $\boldsymbol{b}$, by setting $0.5\leq\theta_{q}\leq1$
% in (\ref{eq:joint_otp_prob}).
%
%\subsubsection*{Varying Quality factor parameter}
%Figure \ref{fig:meanStallVsArrRate} 
% shows the average quality of the streamed videos versus the
%stall factor $\theta_{s}$ for the selected set of algorithms. Apparently,
%our proposed approach gives the highest quality as it aggressively
%maximizes the quality over the stall duration, i.e., streaming the
%larger videos by the highest possible probability. These results show
%also the greedy behavior of our proposed approach as $\theta_{q}$  increases (or alternatively $\theta_{s}$ decreases) and clearly at $\theta_{q}=1$ (that is, $\theta_{s}=0$) our approach streams the video of the largest size and thus the average quality of the streamed video is
%$\ell=6$, i.e., which is the highest possible quality. 


%\begin{figure}[t]
%		\centering
%		\includegraphics[trim=0.1in 0in 0.0in 0.1in, clip, scale =0.30]{figs/stall_vs_vidSize_all}
%		\vspace{-.2in}
%		\captionof{figure}{Mean stall duration for different video lengths.}
%		\label{fig:meanStallVsVidSize} 
%		\vspace{-.18in}
%	\end{figure}%












%\begin{figure*}
%	\centering
%	\begin{minipage}{.32\textwidth}
%		\centering
%		\includegraphics[trim=0.1in 0in 5in 0in, clip, width=\textwidth]{figs/qlty_vs_vidSize_all}
%%		\vspace{-.3in}
%		\captionof{figure}{Average streamed quality for different video lengths.}
%		\label{fig:meanQltyVsVidSize}
%	\end{minipage}%
%	\hspace{2mm}
%	\begin{minipage}{.32\textwidth}
%		\centering
%		\includegraphics[trim=0.1in 0in 5in 0in, clip, width=\textwidth]{figs/qlty_stall_vs_d_j2}
%%		\vspace{-.3in}
%		\captionof{figure}{Average video quality and mean stall duration for different number of parallel streams $d_j$.}
%		\label{fig:qlty_stall_Vs_d_j}
%	\end{minipage}
%	\hspace{2mm}
%	\begin{minipage}{.32\textwidth}
%		\centering
%		\includegraphics[trim=0in 0in 5in 0in, clip,width=\textwidth]{figs/tradeOff}
%%		\vspace{-.3in}
%		\captionof{figure}{Tradeoff between mean stall duration and  average streamed video quality obtained by varying $\theta$.}
%		\label{fig:tradeoff} 
%	\end{minipage}
%%	\vspace{-.2in}
%\end{figure*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


















%\begin{figure}[t]
%		\centering
%		\includegraphics[trim=0.1in 0in 0.0in 0in, clip, scale =0.30]{figs/qlty_vs_vidSize_all}
%		\vspace{-.2in}
%		\captionof{figure}{ Average streamed quality for different video lengths.}
%		\label{fig:meanQltyVsVidSize}
%		\vspace{-.18in}
%	\end{figure}
%
%
%	\begin{figure}[t]
%		\centering
%	\includegraphics[trim=0.1in 0in 0.0in 0in, clip, scale =0.35]{figs/qlty_stall_vs_d_j2}
%		\vspace{-.2in}
%		\captionof{figure}{Average video quality and mean stall duration for different number of parallel streams $d_j$.}
%		\label{fig:qlty_stall_Vs_d_j}
%		\vspace{-.18in}
%	\end{figure}





%\begin{figure}[t]
%\includegraphics[scale=0.55]{figures2/Fig_8_stallTail_vs_Num_iterations_source2.eps}
%\caption{Stall duration Tail Probability for different $x$. \label{fig:congStallDiffXvalues} }
%\end{figure}

%\begin{figure}[t]
%\includegraphics[scale=0.55]{figures2/Fig_9_wieghtedLat_vs_x_comp_logy_source.eps}
%\caption{Stall duration tail probability for different $x$ (in seconds). \label{fig:tailProbDiffX} }
%\end{figure}
\subsubsection*{ Effect of the Number of the Parallel Streams ($d_j$)}
Figure \ref{fig:qlty_stall_Vs_d_j} plots the average   streamed video quality and mean stall duration for varying number of parallel streams, $d_j$, for our proposed algorithm. We vary the number of PSs from $10$ to $70$ with increment step of 10 with $\theta=10^{-7}$. Increasing $d_j$ can only improve performance since some of the bandwidth splits can be zero thus giving the lower $d_j$ solution as one of the possible feasible solution. Increasing $d_j$ thus decreases stall durations by having more parallel streams, while increasing average quality. We note that for $d_j<50$, mean stall duration is non-zero and the stall duration decreases significantly while the average quality increases only slightly.  For $d_j>50$, the stall duration remains zero and the average video quality increases significantly with increase in $d_j$. Even though larger $d_j$ gives better results, the server may only be able to handle a limited parallel connections thus limiting the value of $d_j$ in the real systems. 



 %Intuitively, we can see that the stall duration decreases as the number of VMs ($d_j$) increases since more jobs (videos) can be handled (streamed) simultaneously.
 
%  Further, when the mean stall duration is not zero, the proposed algorithm streams the video with approximately base-layer quality as we prioritize the stall minimization over the quality improvement by setting $\theta_q=10^{-7}$. Thus, more videos are concurrently streamed with close to base-layer quality. On contrary, when the mean stall duration is zero, the algorithm starts improving the quality. Hence, the proposed algorithm manages to significantly improve the two QoE metrics as $d_j$ increases. 
%\begin{figure*}
%	\centering
%%	\begin{minipage}{.32\textwidth}
%%		\centering
%%		\includegraphics[trim=0in 0in 0.1in 0in, clip, width=\textwidth]{figs/tradeOff}
%%%		\vspace{-.3in}
%%		\captionof{figure}{Stall duration tail probability for different arrival rates for video files ($x=150$ s).}
%%		\label{fig:tailProbArrRate}
%%	\end{minipage}%
%%		\hspace{2mm}
%%		\begin{minipage}{.32\textwidth}
%%			\centering
%%		\includegraphics[trim=0in 0in 0.1in 0in, clip, width=\textwidth]{figs/convgstall2}
%%%		\vspace{-.3in}
%%		\captionof{figure}{Stall duration tail probability for varying number of video files ($x=150$ s).}
%%		\label{fig:Fig_9_stallLat_vs_NumOfFiles}
%%		\end{minipage}
%%		\hspace{2mm}
%		\begin{minipage}{.32\textwidth}
%			\centering
%			\includegraphics[trim=0in 0in 0.0in 0in, clip,width=\textwidth]{figs/tradeOff}
%	%		\vspace{-.3in}
%			\captionof{figure}{Tradeoff between mean stall duration and stall duration tail probability obtained by varying $\theta$.  }
%			\label{fig:tradeoff}
%		\end{minipage}
%	
%		\vspace{-.2in}
%\end{figure*}

%\begin{figure}[t]
%	\centering
%			\centering
%	\includegraphics[trim=0.1in 0in 0.0in 0in, clip, scale =0.35]{figs/tradeOff}
%			\vspace{-.2in}
%			\captionof{figure}{Tradeoff between mean stall duration and  average streamed video quality obtained by varying $\theta$.}
%			\label{fig:tradeoff}
%			\vspace{-.18in}
%\end{figure}

\vspace{-.05in}
\subsubsection*{Tradeoff  between mean stall duration and  average video quality}


The preceding results show a trade off between the mean stall duration and
the  average quality of the streamed video. In order to investigate such tradeoff, Figure \ref{fig:tradeoff} plots the  average video quality versus the mean stall duration for different values of $\theta$ ranging from $\theta=10^{-8}$ to $\theta=10^{-4}$. This figure implies that a compromise between the two QoE metrics can be achieved by our proposed streaming algorithm by setting $\theta$  to an appropriate value. As expected, increasing $\theta$ will increase the mean stall duration as there is more priority to maximizing the average video quality.   Thus, an efficient tradeoff point between the QoE metrics can be chosen based on the service quality level desired by the service provider. %based on the point on the curve that is appropriate for the clients.

==> sec_5_NumericalResults2.tex <==
\section{Numerical Results}\label{sec:num}
In this section, we evaluate our proposed  algorithm for optimization of mean and tail probability of stall duration and show the effect of the trade-off of parameter $\theta$. We first study the two extremes where only either mean stall duration objective or tail stall duration probability is considered. Then, we show the tradeoff between the two QoE metrics based on the trade-off parameter $\theta$.

%how the impact of the tradeoff objective function varies with respect to the trade-off factor.  



\begin{table}[b]
{\caption{Storage Node Parameters Used in our Simulation (Shift $\beta=10msec$
and rate $\alpha$ in 1/s)}
}


\resizebox{.49\textwidth}{!}{\begin{tabular}{|c|c|c|c|c|c|c|}
\multicolumn{1}{c}{} & \multicolumn{1}{c}{\textbf{Node 1}} & \multicolumn{1}{c}{\textbf{Node 2}} & \multicolumn{1}{c}{\textbf{Node 3}} & \multicolumn{1}{c}{\textbf{Node 4}} & \multicolumn{1}{c}{\textbf{Node 5}} & \multicolumn{1}{c}{\textbf{Node 6}}\tabularnewline
\hline 
{$\alpha_{j}$} & {$18.2298$} & {$24.0552$} & {$11.8750$} & {$17.0526$} & {$26.1912$} & {$23.9059$}\tabularnewline
\hline 
\end{tabular}}

\resizebox{.5\textwidth}{!}{\begin{tabular}{|c|c|c|c|c|c|c|}
\multicolumn{1}{c}{} & \multicolumn{1}{c}{\textbf{Node 7}} & \multicolumn{1}{c}{\textbf{Node 8}} & \multicolumn{1}{c}{\textbf{Node 9}} & \multicolumn{1}{c}{\textbf{Node 10}} & \multicolumn{1}{c}{\textbf{Node 11}} & \multicolumn{1}{c}{\textbf{Node 12}}\tabularnewline
\hline 
{$\alpha_{j}$} & {$27.006$} & {$21.3812$} & {$9.9106$} & {$24.9589$} & {$26.5288$} & {$21.8067$}\tabularnewline
\hline 
\end{tabular}\label{tab:Storage-Nodes-Parameters}
}
\end{table}

\subsection{Numerical Setup}
 We simulate our algorithm in a distributed storage system of $m=12$ distributed nodes, where each video file uses an $(7,4)$ erasure code. We consider $r=1000$ files, whose sizes are generated based on Pareto distribution \cite{arnold2015pareto} with shape factor of $2$ and scale of $300$, respectively. Thus, the first $1000$ file-sizes that are less than 40 minutes are chosen.  We also assume that the chunk service time  follows a shifted-exponential distribution with rate $\alpha_{j}$ and shift $\beta_{j}$, whose values are shown in Table 2, which are generated at random and kept fixed for the experiments. Unless explicitly stated, the arrival rate for the first $500$ files is $0.002s^{-1}$ while for the next $500$ files is set to be $0.003s^{-1}$. Chunk size $\tau$ is set to be equal to $4$ s. When generating video files, the sizes of the video file sizes are rounded up to the multiple of $4$ sec. We note that a high load scenario is considered for the numerical results. In practice, the load will not be that high. However, higher load helps demonstrate the significant improvement in performance as compared to the lightly loaded scenarios where there are almost no stalls. In order to initialize our algorithm, we use a random placement of files on all the servers. Further, we set $\pi_{ij}=k/n$ on the placed servers with $t_{i}=0.01$ $\forall i$ and $j \in \mathcal{S}_{i}$. However, these choices of $\pi_{ij}$ and $t_{i}$ may not be feasible. Thus, we modify the initialization of  $\boldsymbol{\pi}$  to be closest norm feasible solution  given above values of $\boldsymbol{\mathcal{S}}$ and $\boldsymbol{t}$.  We  compare our proposed approach with three strategies:
 \begin{enumerate}[leftmargin=0cm,itemindent=.5cm,labelwidth=\itemindent,labelsep=0cm,align=left]
\item {\em Random Placement, Optimized Access (RP-OA): }  In this strategy, the placement is chosen at random where any $n$  out of $m$ servers are chosen for each file, where each choice is equally likely. Given the random placement, the variables $\boldsymbol{t}$ and $\boldsymbol{\pi}$ are optimized using the Algorithm in Section \ref{sec:algo}, where $\boldsymbol{\mathcal{S}}$-optimization is not performed.

\item {\em Optimized Placement, Projected Equal Access (OP-PEA): }
The strategy utilizes $\boldsymbol{\pi}$, $\boldsymbol{t}$ and $\boldsymbol{\mathcal{S}}$ as mentioned in the setup. Then, alternating optimization over placement and $\boldsymbol{t}$ are performed using the proposed algorithm.

 %In this strategy, the placement is optimized while the access is chosen equally likely at the servers chosen. In order to do that, we perform an iterative algorithm as in Section \ref{sec:algo}, where the $\boldsymbol{\pi}$-optimization is replaced by taking $\pi_{ij}=k/n$ $\forall i$ and $j \in \mathcal{S}_{i}$ and projecting $\boldsymbol{\pi}$ to the feasible set by finding the closest norm feasible solution given above values of $\boldsymbol{\mathcal{S}}$ and $\boldsymbol{t}$.


\item {\em Random Placement, Projected Equal Access (RP-PEA): } In this strategy, the placement is chosen at random where any $n$  out of $m$ servers are chosen for each file, where each choice is equally likely. Further, we set $\pi_{ij}=k/n$ on the placed servers with $t_{i}=0.01$ $\forall i$ and $j \in \mathcal{S}_{i}$. We then modify the initialization of $\boldsymbol{\pi}$ to be closest norm feasible solution  given above values of $\boldsymbol{\mathcal{S}}$ and $\boldsymbol{t}$. Finally, an optimization over $\boldsymbol{t}$ is performed to the objective using Algorithm (\ref{alg:NOVA_Alg1}).


\end{enumerate} 
 
\begin{figure*}[htb]
	\centering
	\begin{minipage}{.32\textwidth}
		\centering
		\includegraphics[trim=0in 0in 0in 0.0in, clip, width=\textwidth]{figs/convgstall2}
		%	\vspace{-.3in}
		\captionof{figure}{Convergence of mean stall duration.}
		\label{fig:ConvgMeanStall}
	\end{minipage}%
	\hspace{2mm}
	\begin{minipage}{.32\textwidth}
		\centering
		\includegraphics[trim=0.0in 0in 0.0in 0in, clip, width=\textwidth]{figs/stall_vs_rate2}
		%	\vspace{-.3in}
		\captionof{figure}{Mean stall duration for different video arrival rates with different video lengths. }
		\label{fig:meanArrRateSameSize}
	\end{minipage}
	\hspace{2mm}
	\begin{minipage}{.32\textwidth}
		\centering
		\includegraphics[trim=0.0in 0in 0.0in 0in, clip,width=\textwidth]{figs/stall_vidSize}
		%		\vspace{-.3in}
		\captionof{figure}{Mean stall duration for different video sizes considering  $\ell=3$.  }
		\label{fig:meanArrRateDiffSize}
	\end{minipage}
	%\vspace{-.2in}
	
	\vspace{-.1in}
\end{figure*}


\subsection{Mean Stall Duration optimization}
In this subsection, we focus only on minimizing the mean stall duration of all files by setting $\theta=1$, {\em i.e.}, stall duration tail probability is not considered.% in this part of the simulation.

\subsubsection*{Convergence of the Proposed Algorithm}
Figure \ref{fig:ConvgMeanStall} shows the convergence  of our proposed algorithm, which alternatively optimizes the mean stall duration of all files over scheduling probabilities $\boldsymbol{\pi}$, auxiliary variables $\boldsymbol{t}$, quality probabilities $\boldsymbol{b}$, and bandwidth allocation weights $\boldsymbol{w}$. We notice that for $r=1000$ video files of size 600 sec with $m=12$ storage nodes and six quality levels shown in \ref{tab:DataRates}, the mean stall duration converges to the optimal value within less than $300$ iterations.  


\subsubsection*{Effect of Arrival Rate} Figures \ref{fig:meanArrRateSameSize}  shows the effect of different video arrival rates on the mean stall duration for different-size video  whose lengths follow the Pareto-distributed described above.  We compare our proposed algorithm with the three baseline  policies and see that the proposed algorithm outperforms all baseline strategies for the QoE metric of mean stall duration. Thus, both access and bandwidth weights allocation of files are both important for the reduction of mean stall duration. We see that the mean stall duration increases with arrival rates. However, our approach still maintain low mean stall duration compared to the baselines.


%Intuitively, having optimized placement leads to less stall duration (for all policies) since video chunks are balanced across the different storage nodes. Hence, the possibility of congested bottleneck nodes reduces accordingly. While mean stall duration increases as arrival rate increases, our approach, unlike PEAP and BNW, does not explode  as others do (especially for optimized one). 

\subsubsection*{Effect of Video Size}
The effect of having different video sizes is also captured in Figure (\ref{fig:meanArrRateDiffSize}). Clearly, larger video sizes may incur more stalls compared to small ones as the chance of getting delayed chunks is increased. However, our proposed approach gives the lowest mean stall duration compared to the considered baselines.
%\begin{figure}[t]
%\includegraphics[scale=0.55]{figures2/Fig_7_mean_stall_NoOfFiles_source.eps}
%\caption{Mean stall duration for different number of video files with different video sizes. \label{fig:meanStallNumFiles} }
%\end{figure}


\subsubsection*{Effect of the Number of Video Files}

Figure \ref{fig:meanStallNumFiles} demonstrates the impact of varying the number of video files from $200$ files to $1000$ files  on the mean stall duration, where the video lengths are generated according to Pareto distribution with the same parameter defined earlier (scale of 300, and shape of 2).  We note that the proposed optimization strategy effectively reduces the mean stall duration and outperforms the considered baseline strategies. Thus, joint optimization over all three variables $\boldsymbol{t}$,  $\boldsymbol{\pi}$,  $\boldsymbol{w}$, and  $\boldsymbol{b}$ helps reduce the mean stall duration significantly.


\subsection{Average Quality  Optimization}

In this subsection, we consider optimizing (magnifying) the quality of the streamed video by maximizing the quality probabilities, $\boldsymbol{b}$, by setting $0.5\leq\theta_{q}\leq1$
 in (\ref{eq:joint_otp_prob}).

\subsubsection*{Varying Quality factor parameter}
Figure \ref{fig:congStallDiffXvalues} 
 shows the average quality of the streamed videos versus the
stall factor $\theta_{s}$ for the selected set of algorithms. Apparently,
our proposed approach gives the highest quality as it aggressively
maximizes the quality over the stall duration, i.e., streaming the
larger videos by the highest possible probability. These results show
also the greedy behavior of our proposed approach as $\theta_{q}$  increases (or alternatively $\theta_{s}$ decreases) and clearly at $\theta_{q}=1$ (that is, $\theta_{s}=0$) our approach streams the video of the largest size and thus the average quality of the streamed video is
$\ell=6$, i.e., which is the highest possible quality. 


\begin{figure*}
	\centering
	\begin{minipage}{.32\textwidth}
		\centering
		\includegraphics[trim=0.0in 0in 0.0in 0in, clip, width=\textwidth]{figs/stall_NoOfVid}
%		\vspace{-.3in}
		\captionof{figure}{Mean stall duration for different number of video files with different video lengths.}
		\label{fig:meanStallNumFiles} 
	\end{minipage}%
	\hspace{2mm}
	\begin{minipage}{.32\textwidth}
		\centering
		\includegraphics[trim=0.0in 0in 0.0in 0in, clip, width=\textwidth]{figs/qualty_vs_theta_q}
%		\vspace{-.3in}
		\captionof{figure}{ Average Streamed Quality versus quality factor $\theta_q$}
		\label{fig:congStallDiffXvalues}
	\end{minipage}
	\hspace{2mm}
	\begin{minipage}{.32\textwidth}
		\centering
		\includegraphics[trim=0in 0in 0.1in 0in, clip,width=\textwidth]{figs/qlty_stall_vs_d}
%		\vspace{-.3in}
		\captionof{figure}{Average Video Quality and Mean Stall duration versus the number of virtual queues $d$}
		\label{fig:tailProbDiffX}
	\end{minipage}
%	\vspace{-.2in}

\vspace{-.15in}
\end{figure*}




%\begin{figure}[t]
%\includegraphics[scale=0.55]{figures2/Fig_8_stallTail_vs_Num_iterations_source2.eps}
%\caption{Stall duration Tail Probability for different $x$. \label{fig:congStallDiffXvalues} }
%\end{figure}

%\begin{figure}[t]
%\includegraphics[scale=0.55]{figures2/Fig_9_wieghtedLat_vs_x_comp_logy_source.eps}
%\caption{Stall duration tail probability for different $x$ (in seconds). \label{fig:tailProbDiffX} }
%\end{figure}
\subsubsection*{ Effect of the Number of the Virtual Queues $d$}
Figure \ref{fig:tailProbDiffX} plots the 
average of the streamed video quality and mean stall duration versus the number of virtual queses $d$. We vary the number of VQs from 5 to 30 with increment step of 5 and we set $\theta_q=1e-6$. We can see that the stall duration decreases as the number of VQs increases since more jobs can be handled simultaneously. We also observe that the proposed algorithm gives higher quality as $d$ increases which results from serving more than a job concurrently and allows for larger videos to be served. Hence, the proposed algorithm manages to significantly improve the two QoE metrics as $d$ increases.

%\begin{figure*}
%	\centering
%%	\begin{minipage}{.32\textwidth}
%%		\centering
%%		\includegraphics[trim=0in 0in 0.1in 0in, clip, width=\textwidth]{figs/tradeOff}
%%%		\vspace{-.3in}
%%		\captionof{figure}{Stall duration tail probability for different arrival rates for video files ($x=150$ s).}
%%		\label{fig:tailProbArrRate}
%%	\end{minipage}%
%%		\hspace{2mm}
%%		\begin{minipage}{.32\textwidth}
%%			\centering
%%		\includegraphics[trim=0in 0in 0.1in 0in, clip, width=\textwidth]{figs/convgstall2}
%%%		\vspace{-.3in}
%%		\captionof{figure}{Stall duration tail probability for varying number of video files ($x=150$ s).}
%%		\label{fig:Fig_9_stallLat_vs_NumOfFiles}
%%		\end{minipage}
%%		\hspace{2mm}
%		\begin{minipage}{.32\textwidth}
%			\centering
%			\includegraphics[trim=0in 0in 0.0in 0in, clip,width=\textwidth]{figs/tradeOff}
%	%		\vspace{-.3in}
%			\captionof{figure}{Tradeoff between mean stall duration and stall duration tail probability obtained by varying $\theta$.  }
%			\label{fig:tradeoff}
%		\end{minipage}
%	
%		\vspace{-.2in}
%\end{figure*}

\begin{figure}[t]
	\centering
%		\hspace{2mm}
		\begin{minipage}{.32\textwidth}
			\centering
			\includegraphics[trim=0in 0in 0.0in 0in, clip,width=\textwidth]{figs/tradeOff}
	%		\vspace{-.3in}
			\captionof{figure}{Tradeoff between mean stall duration and streamed video quality obtained by varying $\theta_s$.  }
			\label{fig:tradeoff}
		\end{minipage}
	
		\vspace{-.2in}
\end{figure}


\subsection{Tradeoff  between mean stall duration and video quality}


The preceding results show a trade off between the mean stall duration and
the streamed quality. In order to investigate such tradeoff, Figure \ref{fig:tradeoff} plots the average video quality versus the mean stall duration for different values of $\theta$ ranging from $\theta=10^{-5}$ to $\theta=10^{-7}$. This figure implies that a compromise between the two QoE metrics can be achieved by our proposed   streaming algorithm by setting the quality and stall factors ($\theta_q$ and $\theta_s$) to proper values. As expected, increasing $\theta_s$ will reduce the mean stall duration as higher priority is giving to minimize the stall over the quality. Thus, an efficient tradeoff point between the QoE metrics can be chosen based on the point on the curve that is appropriate for the clients.



==> subOptProblems.tex <==
\subsubsection{Server-PSs Access Optimization}

Given the bandwidth allocation weights, the cache placement, edge-cache window size, and the auxiliary variables, this sub-problem can be written as follows. 

\textbf{Input: $\boldsymbol{h}$, $\boldsymbol{w}$, $\boldsymbol{\omega}$,  and  $\boldsymbol{L}$}

\textbf{Objective:} $\qquad\quad\;\;$min $\left(\ref{eq:optfun}\right)$

$\hphantom{\boldsymbol{\text{Objective:}\,}}\qquad\qquad$s.t. \eqref{eq:rho_beta_d}--\eqref{eq:pi_q_p_gz}, \eqref{eq:mgf_beta_d}--
\eqref{eq:mgf_beta_e}\\
$\hphantom{\boldsymbol{\text{Objective:}\,}}\qquad\qquad$var. $\widetilde{\boldsymbol{\pi}}$

%Now, we explain our approach in solving $\boldsymbol{\pi}$- Optimization sub-problem. We optimize over $\pi_{ij}$, $\forall i,j$ for given placement $\boldsymbol{\mathcal{S}}$ and fixed $\boldsymbol{t}$. This problem is non-convex as shown in Section \ref{sec:probForm}. Hence, 

In order to solve this problem, we use iNner cOnVex
Approximation (NOVA)  algorithm proposed in \cite{scutNOVA}. The key idea for this algorithm is that the non-convex objective function is replaced by suitable convex approximations at which convergence to a stationary solution of the original non-convex optimization is established. NOVA solves the approximated function efficiently and maintains feasibility in each iteration. The objective function can be approximated by a convex one (e.g., proximal gradient-like approximation) such that the first order properties are preserved \cite{scutNOVA},  and this convex approximation can be used in NOVA algorithm.

Let $\widetilde{U_{q}}\left(\widetilde{\boldsymbol{\pi}},\boldsymbol{\widetilde{\pi}^{\nu}}\right)$ be the
convex approximation at iterate $\boldsymbol{{\pi}^\nu}$ to the original non-convex problem $U\left(\widetilde{\boldsymbol{\pi}}\right)$, where $U\left(\widetilde{\boldsymbol{\pi}}\right)$ is given by (\ref{eq:optfun}). Then, a valid choice of $U\left(\widetilde{\boldsymbol{\pi}};\boldsymbol{{\pi}^\nu}\right)$ is the first order approximation of  $U\left(\widetilde{\boldsymbol{\pi}}\right)$, e.g., (proximal) gradient-like approximation, i.e.,

\begin{equation}
\widetilde{U_{q}}\left(\widetilde{\boldsymbol{\pi}},\boldsymbol{\widetilde{\pi}^{\nu}}\right)=\nabla_{\widetilde{\boldsymbol{\pi}}}U\left(\widetilde{\boldsymbol{\pi}}^{\nu}\right)^{T}\left(\widetilde{\boldsymbol{\pi}}-\widetilde{\boldsymbol{\pi}}^{\nu}\right)+\frac{\tau_{u}}{2}\left\Vert \widetilde{\boldsymbol{\pi}}-\widetilde{\boldsymbol{\pi}}^{\nu}\right\Vert ^{2}
,\label{eq:U_x_u_bar}
\end{equation}
where $\tau_u$ is a regularization parameter. Note that all the constraints \eqref{eq:rho_beta_d}--\eqref{eq:pi_q_p_gz} are separable and
linear in $\widetilde{\pi}_{i,j,k}$.  
 The NOVA Algorithm for optimizing $\widetilde{\boldsymbol{\pi}}$ is described in  Algorithm \ref{alg:NOVA_Alg1Pi} (given in Appendix \refeq{apdx_alg}). Using the convex approximation $\widetilde{U_{\pi}}\left(\boldsymbol{\pi};\boldsymbol{{\pi}^\nu}\right)$, the minimization steps in Algorithm \ref{alg:NOVA_Alg1Pi} are convex, with linear constraints and thus can be solved using a projected gradient descent algorithm. A step-size ($\gamma
$)  is also used in the update of the iterate $\widetilde{\boldsymbol{\pi}}^{\nu}$. Note that the iterates $\left\{ \boldsymbol{\pi}^{\nu}\right\} $ generated by the algorithm are all feasible for the original problem and, further, convergence is guaranteed, as shown in \cite{scutNOVA} and described in   lemma \ref{lem_pi}. 

In order to use NOVA, there are some assumptions (given in \cite{scutNOVA}) that have to be satisfied in both original function and its approximation. These assumptions can be classified into two categories. The first category is the set of conditions that ensure that the original problem and its constraints are continuously differentiable on the domain of the function, which are satisfied in our problem. The second category is the set of conditions that ensures that the approximation of the original problem is uniformly strongly convex on the domain of the function. The latter set of conditions are also satisfied as the chosen function is strongly convex and its domain is also convex. To see this, we need to show that the constraints \eqref{eq:rho_beta_d}--\eqref{eq:pi_q_p_gz} form a convex domain in $\widetilde{\boldsymbol{\pi}}$
 which is easy to see from the linearity of the constraints. Further details on the assumptions and function approximation can be found in \cite{scutNOVA}. Thus, the following result holds. 


\begin{lemma}  \label{lem_pi}
For fixed $\boldsymbol{h}$, $\boldsymbol{w}$, $\boldsymbol{\omega}$,  and  $\boldsymbol{L}$, the optimization of our problem over 
$\widetilde{\boldsymbol{\pi}}$
 generates a sequence of  decreasing
objective values and therefore is guaranteed to converge to a stationary point.
\end{lemma}




\subsubsection{Auxiliary Variables Optimization}
Given the probability distribution of the server-PSs scheduling probabilities, the bandwidth allocation weights, edge-cache window size, and the cache placement, this subproblem can be written as follows. 

\textbf{Input: $\widetilde{\boldsymbol{\pi}}$, $\boldsymbol{w}$, $\boldsymbol{\omega}$,  and $\boldsymbol{L}$ }

\textbf{Objective:} $\qquad\quad\;\;$min $\left(\ref{eq:optfun}\right)$

$\hphantom{\boldsymbol{\text{Objective:}\,}}\qquad\qquad$s.t.  \eqref{eq:t_leq_alpha_beta_d}--\eqref{eq:mgf_beta_e}, \\
$\hphantom{\boldsymbol{\text{Objective:}\,}}\qquad\qquad$var. $\boldsymbol{h}$


Similar to Server-PSs Access Optimization, this optimization can be solved using NOVA algorithm. The constraints  \eqref{eq:t_leq_alpha_beta_d}--\eqref{eq:t_leq_alpha_nu_e} are linear in $\boldsymbol{h}$. Further, the next  Lemma show that the constraints  \eqref{eq:mgf_beta_d}-- \eqref{eq:mgf_beta_e} are convex in $\boldsymbol{h}$, respectively.


\begin{lemma}
%	\label{const68_70}
The  constraints \eqref{eq:mgf_beta_d}--\eqref{eq:mgf_beta_e} are convex with respect to  $\boldsymbol{{h}}$.  \label{cnv_t}
\end{lemma}
\begin{proof}
	The proof is given in Appendix \ref{apd_ww}. 
\end{proof}




 Algorithm \ref{alg:NOVA_Alg1} (given in Appendix \refeq{apdx_alg}) shows the used procedure to solve for $\boldsymbol{h}$. Let $\overline{U}\left(\boldsymbol{h};\boldsymbol{h^\nu}\right)$ be the
convex approximation at iterate $\boldsymbol{h^\nu}$ to the original non-convex problem $U\left(\boldsymbol{h}\right)$, where $U\left(\boldsymbol{h}\right)$ is given by (\ref{eq:optfun}), assuming other parameters constant. Then, a valid choice of  $\overline{U}\left(\boldsymbol{h};\boldsymbol{h^\nu}\right)$ is the first order approximation of  $U\left(\boldsymbol{h}\right)$, i.e.,  
\begin{equation}
\overline{U}\left(\boldsymbol{h},\boldsymbol{h^\nu}\right)=\nabla_{\boldsymbol{h}}U\left(\boldsymbol{h^\nu}\right)^{T}\left(\boldsymbol{h}-\boldsymbol{h^\nu}\right)+\frac{\tau_{h}}{2}\left\Vert \boldsymbol{h}-\boldsymbol{h^\nu}\right\Vert ^{2}.\label{eq:U_t_u_bar}
\end{equation}
where $\tau_h$ is a regularization parameter. The detailed steps can be seen in Algorithm \ref{alg:NOVA_Alg1}. Since all the constraints  \eqref{eq:t_leq_alpha_beta_d}-- \eqref{eq:mgf_beta_e} have been shown to be convex in $\boldsymbol{h}$, the optimization problem in Step 1 of  Algorithm \ref{alg:NOVA_Alg1} can be solved by the standard projected gradient descent algorithm. 

%Similar to Access  Optimization problem, we get the minimizer for (\ref{eq:U_t_u_bar}), step 1 in Algorithm \ref{alg:NOVA_Alg1}), and then continue until convergence. 


%In this sub-problem, we solve for all $t_i$, for fixed placement and given accessing probabilities. Similar to $\boldsymbol{\pi}$- Optimization problem, we used NOVA algorithm to solve for $t$.  Algorithm \ref{alg:NOVA_Alg1}, shows the used procedure to solve for $\boldsymbol{t}$. After initialization with feasible choice, NOVA keeps generating  a sequence of monotonically decreasing $\left\{ \boldsymbol{t}^{\nu+1}\right\} $ until  convergence.

\begin{lemma} \label{lem_t}

For fixed $\widetilde{\boldsymbol{\pi}}$, $\boldsymbol{w}$, $\boldsymbol{\omega}$, and  $\boldsymbol{L}$, the optimization of our problem over $\boldsymbol{h}$ generates a sequence of monotonically decreasing objective values and therefore is guaranteed to converge to a stationary point.
\end{lemma}


\input{w_opt}
\input{L_opt}
\input{omega_opt}

%\input{apdx_algs}

\subsubsection{Convergence of the Proposed Algorithm}

We first initialize 
$\widetilde{\boldsymbol{\pi}}$, $\boldsymbol{w}$, $\boldsymbol{h}$, $\boldsymbol{\omega}$, and $\boldsymbol{L}$ $\forall i, j, \nu_j, \beta_j$ such that the choice is feasible for the problem. Then, we do alternating minimization over the four sub-problems defined above. Since each sub-problem can only decrease the objective and the overall problem is bounded from below, we have the following result.

\begin{theorem} 
 The proposed algorithm  converges to a  local optimal solution.
\end{theorem}
